E-morphic: Scalable Equality Saturation for Structural Exploration in Logic Synthesis

In technology mapping, the quality of the final implementation heavily relies on the circuit structure after technology-independent optimization. Recent studies have introduced equality saturation as a novel optimization approach. However, its efficiency remains a hurdle against its wide adoption in logic synthesis. This paper proposes a highly scalable and efficient framework named E-morphic. It is the first work that employs equality saturation for resynthesis after conventional technology-independent logic optimizations, enabling structure exploration before technology mapping. Powered by several key enhancements to the equality saturation framework, such as direct e-graph-circuit conversion, solution-space pruning, and simulated annealing for e-graph extraction, this approach not only improves the scalability and extraction efficiency of e-graph rewriting but also addresses the structural bias issue present in conventional logic synthesis flows through parallel structural exploration and resynthesis. Experiments show that, compared to the state-of-the-art delay optimization flow in ABC, E-morphic on average achieves 12.54% area saving and 7.29% delay reduction on the large-scale circuits in the EPFL benchmark.

==> algorithms/equality_saturaction.tex <==
\begin{algorithm}[b]
  \caption{Equality Saturation for Optimization}
  \label{eqast_alg}
  \SetAlgoLined
  \SetKwInOut{Input}{Input}
  \SetKwInOut{Output}{Output}

  \Input{Term $\mathcal{T}$, rewrite rules $\mathcal{R}:\{lhs\rightarrow rhs\}$}
  \Output{Optimized term $\mathcal{T}'$}

  \BlankLine
  $\mathcal{E}$ $\leftarrow$ initial\_egraph($\mathcal{T}$)\;
  $iteration \gets 0$
  \BlankLine
  \While{egraph is not saturated and exit condition is not met}{
      \SetCommentSty{textnormal}
      \tcp{exit condition can be set as an upper limit on the iterations or the runtime limit.}
    
    matches $\leftarrow$ \textit{EmptyArray}\;

    \BlankLine

    \For{rw in $\mathcal{R}$}{
      \For{(subst, eclass) in $\mathcal{E}$.ematch(rw.lhs)}{
        matches.append((rw, subst, eclass))\;
      }
    }

    \BlankLine
    \For{(rw, subst, eclass) in matches}{
      new\_eclass $\leftarrow$ $\mathcal{E}$.add(rw.rhs.subst(subst))\;
      $\mathcal{E}$.merge(eclass, new\_eclass)\;
    }
    $iteration \mathrel{+}= 1$
    \BlankLine
    $\mathcal{E}$.rebuild()\;

    
  }
 
  \BlankLine
  \Return $\mathcal{E}$.extract\_best()\;
\end{algorithm}

==> algorithms/extraction_pseudocode.tex <==
\begin{algorithm}
    \caption{Simulated Annealing-based Extraction}
    \label{sa_extraction}
    \SetAlgoLined
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
    
    \Input{An e-graph $\mathcal{E}$, cost function $\mathcal{C}$, initial temperature $T_0$, cooling rate $\alpha$, min temperature $T_{min}$}
    \Output{ExtractionResult $\mathcal{O}_{best}$: best solution found}
    
    $\mathcal{O}_{current} \leftarrow$ GenerateInitialSolution($\mathcal{E}$, $\mathcal{C}$)\;
    $\mathcal{O}_{best} \leftarrow \mathcal{O}_{current}$\;
    $T \leftarrow T_0$\;
    
    \While{$T > T_{min}$}{
      \For{$i \leftarrow 1$ \KwTo $iterations\_per\_temp$}{
        $\mathcal{O}_{new} \leftarrow$ GenerateNeighborSolution($\mathcal{O}_{current}$, $\mathcal{E}$, $\mathcal{C}$, $T$, $T_0$)\;
        $\Delta E \leftarrow$ Cost($\mathcal{O}_{new}$) - Cost($\mathcal{O}_{current}$)\;
        
        \If{$\Delta E \leq 0$ \textbf{or} $random() < e^{-\Delta E / T}$}{
          $\mathcal{O}_{current} \leftarrow \mathcal{O}_{new}$\;
          \If{Cost($\mathcal{O}_{current}$) < Cost($\mathcal{O}_{best}$)}{
            $\mathcal{O}_{best} \leftarrow \mathcal{O}_{current}$\;
          }
        }
      }
      $T \leftarrow \alpha T$\;
    }
    
    \Return $\mathcal{O}_{best}$\;
  \end{algorithm}
  
  \begin{algorithm}
    \caption{GenerateNeighborSolution}
    \label{generate_neighbor_random}
    \SetAlgoLined
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
    
    \Input{Current solution $\mathcal{O}_{current}$, e-graph $\mathcal{E}$, cost function $\mathcal{C}$, random probability $p_{random}$}
    \Output{New solution $\mathcal{O}_{new}$}
    
    $\mathcal{O}_{new} \leftarrow \mathcal{O}_{current}$\;
    $traversalQueue \leftarrow$ InitializeQueueWithLeafNodes($\mathcal{E}$)\;
    $costs \leftarrow$ InitializeCosts($\mathcal{E}$)\;
    
    \While{$traversalQueue$ is not empty}{
      $node \leftarrow traversalQueue$.pop()\;
      $class \leftarrow$ GetClass($node$)\;
      $prev\_cost \leftarrow costs[class]$\;
      $new\_cost \leftarrow \mathcal{C}(node, costs)$ //naive cost model\;
      
      \If{$prev\_cost = \infty$ \textbf{or} ($new\_cost < prev\_cost$ \textbf{and} $random() \geq p_{random}$)}{
        $\mathcal{O}_{new}$.choose($class$, $node$)\;
        $costs[class] \leftarrow new\_cost$\;
        $traversalQueue$.extend(GetParents($class$))\;
      }
    }
    
    \Return $\mathcal{O}_{new}$\;
  \end{algorithm}

==> algorithms/extraction_pseudocode_.tex <==
\begin{algorithm}[!tb]
\caption{Tunable stochastic extraction}
\label{extraction}
\SetAlgoLined
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}

\Input{e-graph $\mathcal{E}$, probability ${K}$, cost function $\mathcal{C}$}
\Output{ExtractionResult $\mathcal{O}$: hashmap of selected e-nodes for each e-class}

$Q \leftarrow$ \{all leaf nodes in $\mathcal{E}$\}\;
$M \leftarrow$ \{ $\infty$ , for all e-classes\}\;

\While{$Q$ not empty}{
$n \leftarrow Q$.deque(); $c \leftarrow n2c(n)$\;
$p \leftarrow M[c]$\;
$CS \leftarrow \text{children of } n$\; 
\uIf{$\mathcal{C}$ is ``sum cost''}{
    $v \leftarrow C(n) + \sum_{i \in CS} M[i]$\;
}
\ElseIf{$\mathcal{C}$ is ``depth cost''}{
    $v \leftarrow C(n) + \max_{i \in CS} \{M[i]\}$\;
}
\If{$v < p$ and $random() \leq 1-K$}{
    $M[c] \leftarrow v$\;
    $Q$.enque($c$.parents)\;
    select $n$ for $c$ and record in $\mathcal{O}$\;
}
}
\Return $\mathcal{O}$
\end{algorithm}

==> algorithms/extraction_pseudocode_bak.tex <==
\begin{algorithm}
  \caption{Tunable stochastic extraction}
  \label{extraction}
  \SetAlgoLined
  \SetKwInOut{Input}{Input}
  \SetKwInOut{Output}{Output}
  
  \Input{An e-graph $\mathcal{E}$, a probability ${K}$, {a cost function $\mathcal{C}$}}
  \Output{ExtractionResult $\mathcal{O}$: a hashmap that records which e-node is selected for each e-class.}
  
  $analysis\_pending\_queue \leftarrow$ \{all leaf nodes in $\mathcal{E}$\}\;
  $Costs\_map \leftarrow$ \{ $\infty$ , for all e-classes\}\;
  \BlankLine
  \While{$analysis\_pending\_queue$ is not empty}{
  $enode \leftarrow $ $analysis\_pending\_queue$.deque();
  
  $eclass \leftarrow enode2eclass(enode)$;
  
  $prev\_cost \leftarrow Costs\_map[eclass]$\;
  
  \BlankLine
  $CS \leftarrow \text{all children of } enode$\; 
  \If{$\mathcal{C}$ is a ``sum cost''}{
      $curr\_cost \leftarrow C(enode) + \sum_{i \in CS} Costs\_map[i]$\;
  }
  \If{$\mathcal{C}$ is a ``depth cost''}{
      $curr\_cost \leftarrow C(enode) + \max_{i \in CS} \{Costs\_map[i]$\}\;
  }
  \BlankLine
  \If{curr\_cost $<$ prev\_cost}{
      \If{random() $\leq {1-K}$}{
          $Costs\_map[eclass] \leftarrow$ $curr\_cost$\;
          $analysis\_pending\_queue$.enque($eclass$.parents)\;
          select $enode$ for $eclass$ and record in $\mathcal{O}$\;
      }
  }
  }
  \Return  $\mathcal{O}$;
  \end{algorithm}

==> deprecated/method_bak.tex <==
% \section{\deftextEsynTurbo}\label{sec:our-method}


\begin{figure*}[t!]
    \centering
    \includegraphics[width=0.9\linewidth]{figs/overview_beta.pdf}
    \caption{\deftextEsynTurbo overview}
    \label{EsynTurbo_overview}
\end{figure*}

\section{\deftextEsynTurbo}\label{sec:our-method}


\guangyu{I am working on this section, please do not modify yet}

%\hongce{Will start to work on this part.}
% \begin{figure*}[thb]
%     \centering
%     \begin{subfigure}{0.49\linewidth}
%         \centering
%         \includegraphics[width=0.8\linewidth]{figs/conv_flow_comp.pdf}
%         \caption{Compare with Conventional Synthesis Flow}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}{0.49\linewidth}
%         \centering
%         \includegraphics[width=0.8\linewidth]{figs/conv_operator_comp.pdf}
%         \caption{Compare with Conventional Optimization Operator}
%     \end{subfigure}
%     \caption{}
%     \label{}
% \end{figure*}

% This section describes our framework \deftextEsynTurbo. Specifically, we will focus on the improvements over the prior  \deftextEsyn framework, 
%and how we conduct a brand-new, more in-depth analysis of integrating equality saturation with existing logic synthesis tools.

%from an overview to the details of high efficient conversion between equation format and e-graph, a combined internal check points runner , faster and better extraction algorithm.

While \deftextEsyn demonstrated the potential of using equality saturation in logic synthesis to avoid local optima caused by destructive logic rewriting, it faces several significant challenges that limit its scalability and efficiency:

\begin{enumerate}
    \item \textbf{Inefficient intermediate representation:} \deftextEsyn uses S-expressions as an intermediate format between the equation format and e-graphs. S-expressions, being nested lists derived from flattening abstract syntax trees (ASTs), are not ideal for representing circuit graphs. As illustrated in Figure~\ref{fig:ast-dag}, shared nodes must be duplicated in S-expressions, leading to significant space and time overhead during circuit-to-e-graph conversion and potentially degrading the overall quality of results (QoR).

    \item \textbf{Scalability issues:} The equality saturation process can grow the e-graph rapidly, especially when applying associative and commutative rules. For large-scale circuits, it becomes impractical to reach saturation in a reasonable time. Previous work, including \deftextEsyn, relied on static termination conditions (e.g., fixed iteration count or runtime limit), which are often suboptimal and hard to set universally across different circuits.

    \item \textbf{Inefficient extraction:} The extraction algorithm in the \texttt{egg} framework, used by \deftextEsyn, doesn't avoid unnecessary work. It recomputes e-node costs even when children nodes haven't changed, leading to significant time overhead, particularly for large-scale circuits.

    \item \textbf{Limited cost functions:} The extraction process in \deftextEsyn primarily uses tree-based cost functions (e.g., AST size and depth), which may not accurately reflect the QoR of circuit graphs.
\end{enumerate}

These challenges highlight the need for a more efficient and scalable approach to e-graph-based logic synthesis. Our work, \deftextEsynTurbo, addresses these issues by introducing several key improvements, which we will discuss in the following sections.

\guangyu{This section describes our framework \deftextEsynTurbo. Specifically, we will focus on the improvements over the prior  \deftextEsyn framework,
and how we conduct a brand-new, more in-depth analysis of integrating equality saturation with existing logic synthesis tools.
}

\subsection{Framework Overview}


% \begin{figure*}[thb]
%     \centering
%     \includegraphics[width=0.9\linewidth]{figs/overview_beta.pdf}
%     \caption{\deftextEsynTurbo overview}
%     \label{EsynTurbo_overview}
% \end{figure*}

%\guangyu{TODO: modify this part according to the modified flow chart}
% \begin{figure}[bt]
%     \centering
%     \includegraphics[width=0.5\textwidth]{figs/esynturbo_simple.pdf}
%     \caption{\deftextEsynTurbo overview}
%     \label{EsynTurbo_overview}
% \end{figure}

\begin{figure}[b]
    \centering
    \includegraphics[width=0.49\textwidth]{figs/SA.pdf}
    \caption{SA extraction algorithm}
    \label{fig:SA}
\end{figure}





\guangyu{\ref{} illustrates a high-level overview of the \deftextEsynTurbo flow for logic synthesis. Its new features are summarized as follows:
%\cchen{workflow fig ---> show how to integrate eqsat for structural refinement for mapping results}
\begin{itemize}
\item Before employing the \deftextEsynTurbo, the input combinational circuit will be optimized by applying conventional synthesis flow in \blackcircled{1}.
\item \deftextEsynTurbo applies an efficient DAG-to-DAG conversion between e-graphs and circuits, tremendously reducing the overhead of using S-expression as the bridge between e-graphs and circuits. We put forward a domain-specific language (DSL) embedded in JSON to support efficient parsing and serialization, which will be elaborated in \S\ref{}.
%\item Unlike \deftextEsyn, in \circled{1} pre-processing and  \circled{4} post-processing, \deftextEsynTurbo does not use the S-expression as the bridge between e-graphs and circuits due to its high overhead. Instead, we put forward a domain-specific language (DSL) embedded in JSON to support efficient mutual conversion, bringing about orders of magnitude speed-up. \looseness=-1
%The input combinational circuit is transformed into an equation format using the logic synthesis tools ABC. We transform the equation format into an intermediate language that can be efficiently parsed into an initial e-graph.
\item A efficient DSL embedded in JSON for circuit---e-graph conversion has been proposed in \blackcircled{2}. This method can be applied to other E-graph based optmization tools, as a replacement of S-expression.
\item \deftextEsynTurbo enhances \blackcircled{3} the extraction method with QoR evaluation procedure, and employs a simulated annealing algorithm for more efficient e-graph extraction.
% \item We develop \circled{2} a dynamic monitoring runner that allows sampling the quality of optimization within rewriting iterations. 
%This integration of rewriting and extraction is enabled by the improved efficiency in the foundational components (e.g.,  extraction and post-processing). 
%Thanks to the improved efficiency in extraction and post-processing, we can now integrate more tightly the rewriting process with the extraction process. Specifically, we develop a dynamic monitoring runner that allows sampling the quality of rewriting in the middle of rewriting iterations. 
%It offers a useful probe into rewriting and helps intelligently set flexible termination conditions per design. \looseness=-1
\item \blackcircled{3} apply golden model and ML model to balance the trade-off between algorithm runtime and synthesis result quality, which will be elaborated in \S\ref{}.
\item Multi-threading is applied in \blackcircled{3} to further reduce the runtime of extraction, making this method more scalable.
\item After the extraction phase on \blackcircled{3}, a combination equivilance checking using \textit{cec} in Bekeley ABC will be applied to confirm the correctness of the extracted result, as shown in \blackcircled{4}.
% \item Given the high-level freedom of configuration in the underlying components, we devise two operation modes for \deftextEsynTurbo:  runtime-oriented mode (using an \textit{Early-Stop Strategy}) and QoR-oriented mode (using an \textit{Exploration Strategy}). These two modes are characterized by different parameters in extraction and the dynamic monitoring runner, targeting faster speed or larger design space exploration, respectively.
%Faster and better extraction algorithms characterized by increased speed and superior performance with tunable tree-based cost function and DAG-based cost function.
%\item The optimized e-graph is transformed back into an equation format from the intermediate language efficiently. The equations can be readily evaluated of delay and area metrics by logic synthesis tools ABC. 
%\item We develop a dynamic monitoring runner that integrates the extraction process into the rewriting process. This runner can record intermediate optimal results in parallel, allowing operation in runtime mode with an \textit{Early-Stop Strategy} or in quality mode with tunable tree-based and DAG-based extraction.\looseness=-1
\end{itemize}
We will elaborate on each point in the following subsections.
}

% \todo{To summarize ...} % summary
% \begin{figure*}[h]
%     \centering
%     \includegraphics[width=\textwidth]{figs/overview_esynturbo_NEW.pdf}
%     \caption{\deftextEsynTurbo overview}
%     \label{EsynTurbo_overview}
% \end{figure*}
% \todo{put the complete equation format in figureshare (just like https://arxiv.org/pdf/2303.01839.pdf}
% \input{tables/rewrite_rules_table}
%  \begin{figure}[t]
%     \centering
%     \begin{subfigure}{0.49\linewidth}
%         \centering
%         \includegraphics[width=0.8\linewidth]{figs/parse_ast.pdf}
%         \caption{Abstract Syntax Tree (AST)}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}{0.49\linewidth}
%         \centering
%         \includegraphics[width=0.8\linewidth]{figs/parse_dag.pdf}
%         \caption{Directed Acyclic Graph (DAG)}
%     \end{subfigure}
%     \caption{Duplication in ASTs (as well as S-expressions) vs. DAG encoding for circuit---e-graph conversion.}
%     %Size comparison on S-expression vs. DAG encoding for circuit to E-Graph conversion}
%     \label{fig:ast-dag}
% \end{figure}

% \begin{figure}[thb]
%     \centering
%     \includegraphics[width=0.49\textwidth]{figs/efficient_conversion.pdf}
%     \caption{Efficient e-graph---circuit conversion}
%     \label{fig:conversion}
% \end{figure}

\begin{figure}[H]
    \vspace*{\fill}
    \hfill
    \begin{minipage}{0.49\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figs/efficient_conversion.pdf}
        \caption{Efficient e-graph---circuit conversion}
        \label{fig:conversion}
    \end{minipage}
\end{figure}

\subsection{Efficient E-Graph Initialization} 
\label{sec:conversion}
%\guangyu{Fix the paragraph headings}
~\newline

\guangyu{
\newline
\indent \textit{1) Backgrounds:} Previous work~\cite{} use S-expression as the intermediate representation, which limit the scalability of the framework. S-expression essentially is a nested list, 
resulting from flattening an abstract syntax tree (AST). It is less convenient when representing a circuit graph. As Figure~\Cref{fig:conversion} shows,
 S-expression will result in exponential growth of the expression size, resulting in a notable space and time overhead in the conversion between circuits and e-graphs, and also deteriorating the overall QoR. 
 In comparision, DAG is a more efficient representation for circuits, as it does not double-count the shared nodes and may better reflect the actual optimization target.
}

%\indent \textit{1) Backgrounds:}~\deftextEsyn uses the intermediate language S-expression as a bridge between the equation format and e-graph in \blackcircled{1} pre-processing and \blackcircled{4} post-processing. However, an S-expression essentially is a nested list, resulting from flattening an abstract syntax tree (AST). It is less convenient when representing a circuit graph. As Figure~\ref{fig:ast-dag} shows, in order to fit into the format, shared nodes have to be duplicated, resulting in a notable space and time overhead in the conversion between circuits and e-graphs, and also deteriorating the overall QoR. 


As mentioned earlier, S-expression could incur significant overhead due to duplication in the list. For example, below is the S-expression for a Boolean logic, where the red color indicates such a duplication. 
\begin{center}
{{\texttt{( + ( + \textcolor{red}{( * a b )} ( * a c )) \textcolor{red}{( * a b )})}}\xspace}
\end{center}

In this example, \texttt{(* a b)} is the common sub-expression that is referred to by multiple parents. However, in general, the common sub-expression (sub-graph) could be very large, resulting in a huge amount of duplication in the S-expression. 

\indent \textit{2) Approach:} we work out a more efficient intermediate format as the bridge of conversion, which is essentially a serialization of the initial e-graph.
 %using \texttt{id} to .
   An example is shown in \Cref{fig:circuit2egraph}. For an equation format input, each assignment corresponds to a node in the initial e-graph, which is referred to by \texttt{id} in the DSL.
In pre-processing, circuits in the equation format are first converted into this DSL, from which a parser that we build constructs the initial e-graph.
In post-processing, \deftextEsynTurbo serializes the extracted e-graph into this DSL and we build another parser to convert it node-by-node into assignments in the equation format.
This methods can be adopted to other E-graph based circuit optmization tasks, benefiting whole EDA community.
% Later, the experiment in \Cref{exp:preprocess} shows that this improvement brings about order-of-magnitude speed-up compared to using S-expressions, enabling \deftextEsynTurbo to tackle much larger circuits.
\begin{figure}[thb]
    % \vspace{-2em}
    \centering
    \frame{\includegraphics[width=0.99\linewidth]{figs/DSL_initial_circuit2egraph.pdf}}
    \caption{The intermediate format for efficient e-graph---circuit conversion in pre- and post-processing.}
    \label{fig:circuit2egraph}
\end{figure}


% By traversing each line of the equation format only once, it is possible to directly build the initial egraph. This is because each line appears in the form "lhs = (!)var0 operator (!)var1", and by using a hashmap, we can record the corresponding mapping between variables in the equation format and the initial enodes.Iteratively add these new enodes to build  an intial e-graph in a defalut language, \cchen{ need a refinement and a example}.Then, we use the Rust serde$\_$json library to convert the egraph into a json file. Processing the json file in a format compatible with a defined boolean language, a intial e-graph could be efiiciently built dircetly from the processed json file.


% \textcolor{blue}{We have developed a new DSL (domain-specific language) for converting circuits and egraphs. This technique greatly enhances the scalability of our framework. With the new DSL, \textit{egg} no longer needs to read S-Expressions as input. As digital circuits are naturally DAGs, the input space can be compressed, allowing the framework to parse large circuits quickly.} 

% \textcolor{blue}{Firstly, we convert the circuit into Synopsys Equation Format by the method proposed in~\cite{chen2024syn}, in this format, circuit is represented in a bit-level connection format. It has three component, which is \textit{input port}, \textit{output port} and \textit{wire (connection relation)}. Thus, this can be interpreted as a DAG, all wire can be encode as the intermediates nodes in the graph. The equation format will be converted to a json as~\Cref{fig:circuit2egraph-before-saturacted} shows, all the nodes will be assigned a unique id, and the boolean operators will also been encoded as nodes. The id followed by the operator can be treated as a subgraph id, if this sub-graph is re-used, the id will be pointed as the children nodes. We using hash technique to assign all the sub-graph (represented the sub-expression) a unique id, the concat operator stands for the output, which is used to make sure it has a only one output, the concat operator will not include any boolean rewriting rules.}

% \textcolor{blue}{The format in~\Cref{fig:circuit2egraph-before-saturacted} it can be easily convert into e-graph with much less efforts than parsing in S-Expression and the sub-expression can be easily re-used, avoiding the input unfold-exploring problem mentioned in~\cite{chen2024syn}. \textit{egg} supports to read this similar format as serialize egraph, thus it can easily rebuild a egraph on this by using \textit{egg::EGraph<Prop, ()> = serde\_json::from\_str}. The DSL has close relation with the defined language.}

% \textcolor{blue}{\Cref{fig:circuit2egraph-after-saturacted} illustrates the E-Graph after saturation. The e-node is represented as the index followed decimal point. Since the saturated graph will contain multiple e-nodes in a e-class, thus this~\Cref{fig:circuit2egraph-after-saturacted} only illustrated a part of saturated e-class 378. The assigned cost is pre-defined in re-writing process. Our framework will perform extraction after this saturated graph. }

% \textcolor{blue}{We have another parser to parse the~\Cref{fig:circuit2egraph-after-saturacted} and convert it back to equation format by recursively parsing the json format.}

%Here's an example for differentiating AST and DAG in circuit representation for e-graph.
%This is an example of representing this function in equation format:
% \begin{center}
% {{\texttt{(\textcolor{red}{(a * b)} + (a * c)) + \textcolor{red}{(a * b)}}}\xspace}
% \end{center}

%\begin{center}
%\begin{tabular}{l}
%    \texttt{INORDER = a b c;}\\
%    \texttt{OUTORDER = output;}\\
%    \texttt{new\_n0\_ = a * b;}\\
%    \texttt{new\_n1\_ = a * c;}\\
%    \texttt{new\_n2\_ = new\_n0\_ + new\_n1\_;}\\
%    \texttt{output = new\_n2\_ + new\_n0\_;}\\
%\end{tabular}
%\end{center}
%For S-Expression representation, it should be converted as this format, which will cause the expression expanse too long easliy:
%\begin{center}
%{{\texttt{( + ( + \textcolor{red}{( * a b )} ( * a c )) \textcolor{red}{( * a b )})}}\xspace}
%\end{center}

%Note that though the functionality of this circuit is not complicated, the S-Expression representation is easily expensive, and this expansion could be exponentially in the worst case. This hindered the application in large design circuits since in large circuits, there are many nodes (sub-graph, or also known as sub-expression) being re-used, and it is impossible to write them all in S-Expression, which will cause the expression to be too long to tackle in ABC and in \texttt{egg}.

%We have used an intermediate language in \texttt{egg} for converting circuits and egraphs. This technique greatly enhances the scalability of our framework. With the intermediate language, \texttt{egg} no longer needs to read S-Expressions as input. As digital circuits are naturally DAGs, the input space can be compressed, allowing the framework to parse large circuits quickly.

%Firstly, we convert the circuit into Synopsys Equation Format by the method proposed in~\cite{chen2024syn}. In this format, the circuit is represented in a bit-level connection format. It has three components: \textit{input port}, \textit{output port}, and \textit{wire (connection relation)}. Thus, this can be interpreted as a DAG, and all wires can be encoded as intermediate nodes in the graph. The equation format will be converted to a json as~\Cref{fig:circuit2egraph-before-saturacted} shows. All the nodes will be assigned a unique id, and the boolean operators will also be encoded as nodes. The id followed by the operator can be treated as a subgraph id. If this sub-graph is re-used, the id will be pointed to as the children nodes. We use a hash technique to assign all the sub-graphs (represented by sub-expressions) a unique id. The concat operator stands for the output, which is used to ensure it has only one output. The concat operator will not include any boolean rewriting rules.

%The format in~\Cref{fig:circuit2egraph-before-saturacted} can be easily converted into an e-graph with much less effort than parsing in S-Expression, and the sub-expression can be easily re-used, avoiding the input unfold-exploring problem mentioned in~\cite{chen2024syn}. \texttt{egg} supports reading this similar format as a serialized egraph, thus it can easily rebuild an egraph using  serialization feature in \texttt{egg}. The intermediate language has a close relation with the defined language.

%We have another parser to parse the serialized e-graph and convert it back to equation format by recursively parsing the json format.

% \begin{figure}[!t]
%     % \vspace{-2em}
%     \centering
%     \frame{\includegraphics[width=0.99\linewidth]{figs/DSL_initial_circuit2egraph.pdf}}
%     \caption{The intermediate format for efficient e-graph---circuit conversion in pre- and post-processing.}
%     \label{fig:circuit2egraph}
% \end{figure}

% \begin{figure}
%     % \vspace{-2em}
%     \centering
%     \frame{\includegraphics[width=0.8\linewidth]{figs/DSL_saturacted_egraph.pdf}}
%     \caption{Egraph after saturacted. The extracted results will be achieved after extraction, and convert back circuit via another parser}
%     \label{fig:circuit2egraph-after-saturacted}
% \end{figure}
\subsection{Simulated Annealing based Extraction Algorithm}\label{sec:faster extraction}
% \cchen{Section 3.3 and 3.4 need to be reorganized}
% \subsection{An Efficient Extraction-to-Evaluation Process}
% \subsubsection{\textbf{Faster And Better Extraction Algorithm. }}

\begin{figure}[thb]
    \centering
    \includegraphics[width=0.49\textwidth]{figs/neighbor_cost.pdf}
    \caption{Neighbor Cost}
    \label{fig:NC}
\end{figure}

~\newline

\input{algorithms/extraction_pseudocode}

\indent \textit{1) Backgrounds:} \guangyu{Simulated Annealing is a probabilistic technique for solving optimization problems.
It is inspired by the process of heating and cooling in metallurgy, where a material is heated to a high temperature and then slowly cooled to achieve a low-energy state (global minimum).
The algorithm allows for a controlled exploration of the solution space, with the ability to escape local minima and converge to the global minimum.
Extraction in equality saturated graph is proved to be NP-hard~\cite{}, how to balance the exploration and exploitation is the key problem.
We define temperature $T$ to control the balance between exploration and exploitation, can $I$ is the number of iterations, $T_0$ is the initial temperature, $T_f$ is the final temperature, $T_i = T_0 * (1 - \frac{I}{I_{max}})^k$ is the temperature decay function, $k$ is the cooling rate.
The metropolis criterion can be defined as $P(C_{new} \rightarrow C_{old}) = e^{-\frac{C_{new} - C_{old}}{T}}$, which means the probability of accepting the new solution is $e^{-\frac{C_{new} - C_{old}}{T}}$.
}

\indent \textit{2) Approach:} 
\guangyu{We embedded the simulated annealing algorithm into the extraction algorithm. As \Cref{SA} shows, we generate the initial solution at first, and generate the neighbor solution by perturb the current solution.
In every extraction result, we use two cost model to evaluate the new solution. First model is the golden model, which is ABC static library. Second model is the GNN model~\cite{}.
For ML model, we extracted the features list down to predict the QoR: Topology sorting of the node, the depth of the node, and node tyeps.
}

\guangyu{
    We generate the neighbor solution by perturb the current solution, illustrated in \Cref{fig:NC}. We employed a simple strategy to generate the initial cost,
    then labeled the cost of different e-class in the e-graph. For each interation of perturb, we have a possibilities to select the neighbor solution with smaller or equal cost.
    This strategy avoid the whole process stuck in local optimal, and ensure the solution will not be worse than the initial solution.
    In this work, we applied the level as the cost to guide the neighbor solution selection. This stragety can balance the exploration and exploitation to some extent.
}

\guangyu{
    \deftextEsynTurbo improves e-graph extraction with a more efficient  implementation. The extraction method is presented in \Cref{extraction}.
}


The Simulated Annealing Extractor is an advanced extraction method that combines the principles of bottom-up extraction with simulated annealing to efficiently explore the solution space of an e-graph. This hybrid approach aims to overcome local optima and find high-quality circuit representations.

The extractor operates as follows illustrated in \Cref{fig:SA}:

\begin{enumerate}
    \item \textbf{Initialization:} We generate an initial solution using a base extraction method, such as greedy depth-first or random selection.
    
    \item \textbf{Simulated Annealing Loop:} The main loop of the algorithm iteratively improves the solution while gradually decreasing the temperature parameter. At each iteration:
    \begin{itemize}
        \item We generate a neighbor solution using a random extraction method, which is illustrated in \Cref{fig:NC}.
        \item We evaluate the cost of the new solution using our cost models, explained in section \ref{sec:cost_model}.
        \item We accept or reject the new solution based on the cost difference and current temperature, allowing for occasional uphill moves to escape local optima.
        \item The whole process is multi-threaded, which means we have multiple agents to evaluate the cost of the new solution in parallel.
    \end{itemize}
    
    \item \textbf{Neighbor Generation:} The random extraction method for generating neighbor solutions works as follows, which is illustrated in \Cref{fig:NC}:
    \begin{itemize}
        \item Start from leaf nodes and propagate changes upwards through the e-graph, blue nodes stands for selected nodes.
        \item For each node, decide whether to update its selection based on a combination of cost improvement and random chance, we only will select the node with local optimal cost, this code is simply use node level as measurement.
        \item This randomness allows for exploration of different parts of the solution space, but still ensure the solution will not be worse than the initial solution.
    \end{itemize}
    
    \item \textbf{Termination:} The algorithm terminates when the temperature reaches a predefined minimum value or after a fixed number of iterations.
\end{enumerate}

\subsection{Cost Models}

We employ two cost models to evaluate the quality of extracted circuits:

\subsubsection{Golden Cost Model (ABC)}
\begin{itemize}
    \item We convert the extracted circuit representation to an equation file (.eqn).
    \item The equation file is processed using the ABC tool, which performs the following steps:
    \begin{itemize}
        \item Read the equation file and a standard cell library.
        \item Perform structural hashing and technology mapping.
        \item Apply post-processing optimizations (topological sorting, gate sizing).
    \end{itemize}
    \item ABC then calculates the circuit delay, which serves as our primary cost metric.
\end{itemize}

\subsubsection{Machine Learning (ML) Cost Model}
\begin{itemize}
    \item We generate feature representations of the circuit using ABC's edge list (.el), feature (.csv), and JSON outputs.
    \item These features are sent to a gRPC server hosting our trained ML model.
    \item The ML model predicts the circuit delay based on the input features.
    \item This prediction serves as an alternative, potentially faster cost estimate.
\end{itemize}

\subsection{Integration of Cost Models}

The two cost models are integrated into our extraction process as follows:

\begin{enumerate}
    % \item During the simulated annealing loop, we primarily use the ABC cost model to evaluate solutions. This ensures high accuracy in our optimization process.
    \item We have two modes to integrate the cost model: First is the runtime-prioritized mode, where the ML cost model is used as a rapid estimation tool, particularly useful for quick evaluations of many candidate solutions, this can providing fast estimates to guide the acceptance probability in the simulated annealing process.
    \item Second is the quality-prioritized mode, where the golden model is used to evaluate the quality of the solution. We combine a static-linked library in abc and using FFI to call the library in Rust.
    % \item The ML cost model is used as a rapid estimation tool, particularly useful for quick evaluations of many candidate solutions. It can be employed in the following scenarios:
    % \begin{itemize}
    %     \item Initial filtering of neighbor solutions before detailed ABC evaluation.
    %     \item Providing fast estimates to guide the acceptance probability in the simulated annealing process.
    % \end{itemize}
    
    % \item We periodically compare the ML model predictions with ABC results to ensure the ML model remains calibrated throughout the extraction process.
\end{enumerate}

By combining these components, our Simulated Annealing Extractor aims to efficiently navigate the complex solution space of e-graphs, leveraging both accurate circuit simulation (ABC) and rapid machine learning-based estimation to find high-quality circuit representations. The use of random extraction in neighbor generation allows for a broader exploration of the solution space, potentially discovering diverse circuit configurations that might be missed by more deterministic approaches.

% As already studied in the prior work~\cite{chen2024syn}, it is in general beneficial to use a combination of minimal tree-based cost (e.g., AST depth or AST size) and random selection to first form a pool of candidates. 
% The probability used for random selection is also configurable, as the difficulty of getting out local minima in different designs varies, and we sometimes need to encourage a more exploratory random walk using a higher random probability. 
% This was called the \textit{pool extraction} method in the prior work. However,the extraction algorithm in~\cite{chen2024syn} does not avoid unnecessary work where an e-node cost is recomputed even though its children have not changed.
% As a result, this inefficient process can lead to notable time overhead, particularly in large-scale circuits.

% \deftextEsynTurbo further develops this idea into \textit{tunable stochastic extraction}, where the cost metric could be either tree-based or DAG-based, or both (note that multiple cost functions can be used in combination and their composition is also one parameter to tune).
% In general, DAG sizes differ from AST sizes as the former do not double-count the shared e-nodes and may better reflect the actual optimization target. 

\guangyu{below is the explanation of the pseudocode}

\deftextEsynTurbo improves e-graph extraction with a more efficient implementation. The extraction method is presented in \Cref{extraction}.
It utilizes a pending queue to record the e-nodes to analyze. The process starts from the leaf e-nodes in the input e-graph $\mathcal{E}$ (\Cref{line:start}). Then, it iterates over each e-node in the pending queue to calculate whether its current cost is smaller than the previously recorded minimum of this e-class. The minimum cost of each e-class is maintained by a hashmap called ``$costs$" (defined in \Cref{line:hashmap}). The current cost is calculated using the input cost function $\mathcal{C}$. Depending on the optimization target, $\mathcal{C}$ may be a ``sum cost'' (such as AST size) or a ``depth cost'' (such as AST depth), which are handled differently as shown in Line~\ref{line:cost_start}-\ref{line:cost_end}.

For a smaller current cost, RandomExtraction updates the record following a random probability $1 - random\_prob$. A higher $random\_prob$ means more exploration of those locally sub-optimal choices, which may be overall beneficial in reaching a global optimal point. Specifically, if the previous cost is infinity (indicating an unvisited node) or if a random value is greater than or equal to $random\_prob$ and the new cost is less than the previous cost, the algorithm updates the extraction result and propagates the change to parent nodes.

Overall, this algorithm selectively visits e-nodes with the potential for cost improvement, leveraging caching (``$costs$") to record optimal costs per e-class. This approach avoids redundant computations by preventing the re-evaluation of e-node costs when the costs of their child nodes remain unchanged. The randomization factor allows for exploration of potentially suboptimal local choices that may lead to better global solutions.
% \deftextEsynTurbo improves e-graph extraction with a more efficient implementation. The extraction method is presented in \Cref{extraction}.
% It utilizes a pending queue to record the e-nodes to analyze. The process starts from the leaf e-nodes in the input e-graph $\mathcal{E}$ (\Cref{line:start}). Then, it iterates over each e-node in the pending queue to calculate whether its current cost is smaller than the previously recorded minimum of this e-class. The minimum cost of each e-class is maintained by a hashmap called "$Costs\_map$" (defined in \Cref{line:hashmap}). The current cost is calculated using the input cost function $\mathcal{C}$. Depending on the optimization target, $\mathcal{C}$ may be a ``sum cost'' (such as AST size) or a ``depth cost'' (such as AST depth), which are handled differently as shown in Line~\ref{line:cost_start}-\ref{line:cost_end}.
% For a smaller current cost, stochastic extraction updates the record following a random probability $K$. A higher $K$ means more exploration of those locally sub-optimal choices, which may be overall beneficial in reaching a global optimal point.

% Overall, this algorithm selectively visits e-nodes with the potential for cost improvement, leveraging caching ("$Costs\_map$") to record optimal costs per e-class. This approach avoids redundant computations by preventing the re-evaluation of e-node costs when the costs of their child nodes remain unchanged.
%As for the implementation, we make use of the \texttt{serde} library in Rust to connect it to interface with the original \texttt{egg} library.
%\hongce{Add implementations ...}
% the cost function for an  equality saturation framework is typically tree-based or integer-linear-programming-based (ILP-based). However, neither is efficient and accurate for DAG-based targets that are common in logic optimization; \hongce{ do we want to emphasize (3) or maybe remove (3)?}\cchen{yes we wanna weaken the importance of 3 }
%\hongce{Will work on this subsection}
%We build an interface, utilizing Rust's serde library, that connects the rewriting runner in the egg framework to a new extraction library - extraction gym\footnote{https://github.com/egraphs-good/extraction-gym} . Inspired by faster bottom-up in extraction gym , We designed a tunable tree-based extraction algorithm in Algorithm~\ref{extraction}:
%%%%%%%%%
%It utilizes a pending queue to record the  ${enodes}$ to analyze. The process starts from the leaf $enodes$ in the $egraph$ $\mathcal{E}$ (Line 1). Then, it iterates over each $enode$ in the pending queue to calculate whether the current cost of the $enode$ is smaller than the previously recorded minimum cost in this $eclass$. The minimum cost of each $eclass$ is maintained by a hashmap called "$Costs\_map$". The current cost is calculated using the input cost function $\mathcal{C}$. Depending on the optimization target, $\mathcal{C}$ may be a ``sum cost'' (such as AST size) or a ``depth cost'' (such as AST depth), which are handled differently as in Line 8-13.
%For a smaller current cost, stochastic extraction updates the record following a random probability $K$. A higher $K$ means  more freedom to explore those sub-optimal candidates, which is beneficial in 

%If $\mathcal{C}$ is set to "node\_sum\_cost," it will sum up the costs of all the children of the current $enode$ and the cost of the current $enode$ itself. If $\mathcal{C}$ is set to "node\_depth\_cost," it will sum up the cost of the current $enode$ and the maximum cost among its children.(Line 13-18).Next, if the current $enode$'s cost is smaller than the previously recorded minimum cost for its corresponding eclass in $Costs\_map$, this $enode$ will be temporarily selected as the extraction result for that $eclass$. Additionally, the minimum cost record for that $eclass$ will be updated with the cost of the current $enode$. Furthermore, all parent $enodes$ of the current $enode$ will be added to the pending queue for further processing. If the random option is enabled, the algorithm will skip the selection of current optimal enode based on a random probability determined by the input random probability ${K}$ (Line 19 -23). Overall, this algorithm selectively visits $enodes$ with the potential for improved cost, leveraging caching to record optimal costs within  $eclass$. This approach avoids redundant computations by preventing the re-evaluation of $enode$ costs when the costs of their child nodes remain unchanged. Additionally, if extended extraction time is accepted, our interface allows for a DAG-based cost function in the extraction gym for further optimization.
% from an \textbf{efficiency} perspective, it utilizes caching to record the current optimal cost and the corresponding selected e-node for each e-class. This algorithm selectively visits only those e-nodes whose current cost estimate has the potential to improve, resulting in a significant reduction in computational cost.\cchen{compare with the worst case show the improvement?} From a \textbf{quality} perspective, it enables the random selection of certain e-nodes with suboptimal costs by incorporating a probability factor ${K}$.
% Although technology-independent optimization heavily relies on graph size and depth metrics and significantly impacts circuit optimization, it cannot guarantee precise optimization of the corresponding delay area after technology mapping. Therefore, our approach, which enables random selection, efficiently preserves suboptimal solutions, which can help explore
% and potentially discover better solutions. In addition, our interface allows for the utilization of a DAG-based extraction cost function in the extraction gym. If sacrificing runtime is acceptable, utilizing DAG size cost function for area optimization can yield better results compared to a tree-based cost metric.


% and dag-based extraction cost function to store multiple solutions for performance-oriented optimization. In addition, our interface allows for the utilization of a DAG-based extraction cost function in the extraction gym. 
% \vspace{-2em}

% with Checkpoints
% \subsubsection{A Dynamic Monitoring Runner}\label{sec:dynamic runner}
% ~\newline
% % Conversely,  The most challenging aspect is that To address this issue, we devise an algorithm in the rewriting runner that allows for setting a fixed number of rounds to detect if the desired optimization objectives have been achieved. However, if the objectives are not met, the runner will continue rewriting until it reaches the maximum time limitation.
% \textbf{1}) Backgrounds:  The Equality Saturation inherently faces an unavoidable challenge since it will never saturate when applying the associativity and commutativity rules ~\cite{termination_eqsat}. These rules lead to rapid growth in the size of the e-graph. Consequently, determining the optimal number of iterations for the rewriting runner becomes
% crucial as it significantly impacts both the quality and speed of the rewriting process. However, \deftextEsyn~\cite{chen2024syn} and all previous work~\cite{coward2022automatic,chen2024syn,cheng2023seer,ustun2022impress,coward2023datapath,ESFO} only utilized a static (pre-determined) termination condition, such as a fixed number of iterations or a fixed runtime limit, which is often hard to set and can have a significant negative impact on both the rewriting speed and optimization performance.

% \textbf{2}) Approach: \deftextEsynTurbo introduces a novel approach that combines e-graph rewriting and extraction processes into a unified dynamic monitoring runner with checkpoints. Thanks to the adoption of faster extraction algorithms in \Cref{sec:faster extraction}, as well as the efficient conversion between e-graphs and equation formats in \Cref{sec:conversion}, we can set checkpoints in the runner process with very low time cost.  The rewriting runner operates on a set interval of ${M}$ iterations. At the end of each interval, it dumps the current e-graph $\mathcal{E'}$  and conducts an extraction based on given cost function(s) to derive an optimal e-graph $\mathcal{E^*}$.
% %Note that, for extraction, multiple cost functions can be used, and the composition of this combination is one parameter to configure.
% The runner can evaluate the optimality of $\mathcal{E^*}$ using post-processing to get a QoR report and meanwhile continue to further rewrite $\mathcal{E'}$. 
% Taking these intermittent objective-oriented evaluations as references,
% this runtime monitoring approach facilitates the runner to control the rewriting process more flexibly.

% Furthermore, we introduce an \textit{Early-Stop Strategy}, which looks at the QoR of consecutive $T$ intervals in a sliding window to detect any signs of improvement. If there is a consistent trend of improvement observed within the window, the algorithm moves on to the next set of intervals without interruption. However, if a result within the current window is no better than the best result identified across all prior recorded ones, this is taken as an indication of a local minimum. Upon recognizing such a local minimum, the \textit{Early-Stop Strategy }terminates the runner and returns the current best result.
% % Regarding the extraction cost in this mode, we use a tree-based cost function with zero randomness to expedite extraction.
% In contrast to the previous approach of setting termination conditions statically, our runner with the \textit{Early-Stop Strategy} not only saves significant runtime during the rewriting and extraction processes but also ensures the preservation of the optimal solution.\cchen{sampling}
% Specifically, we devise two strategies for the rewriting running that target either faster optimization or better quality:\hongce{TODO}


% \textbf{Runtime-oriented mode:} For this mode, 


% \textbf{Quality-oriented mode:} In the quality-oriented mode, we opt for a different strategy. Instead of frequent intervals as in the runtime-oriented mode, we select a set of fixed checkpoints spaced far apart, such as at iterations [3, 30, 60, 90]. This strategy is designed to explore solutions that are distributed across various regions of the solution space, aiming to uncover a broader spectrum of potential optima. At each checkpoint, we use the stochastic tree-based cost functions in combination with the DAG-based ones, and the probability factor $K$ ranges from 0 to 0.3.  
% This process generates $N$ groups of samplings through random extraction in parallel, and significantly increases the variation in the solution space, allowing for greater exploration of different possibilities.  \cchen{remove }

%\hongce{todo: a summary of this section}
% In summary, \deftextEsynTurbo brings about improvements over the key components in an equality saturation framework and takes into account the necessary balance between runtime and quality.

%\textbf{Runner in runtime mode :} The rewriting runner operates on a set check interval of ${M}$ iterations, At each interval, it dumps the current e-graph $\mathcal{E'}$ and conducts an extraction based on the cost function of $\mathcal{E'}$ to derive an optimal e-graph after extraction $\mathcal{E^*}$, while also temporarily storing $\mathcal{E^*}$. Additionally, at every $T$ check intervals, a check point is taken. For the cost function, with the aim of optimizing runtime, we have selected a tunable tree-based extractor that excludes randomness. Then our runner transform these $T$ temporarily stored $\mathcal{E^*}$ in parallel into equation format using the efficient back-end parser. Finally, the logic synthesis tool ABC is utilized to obtain their delay and area in parallel. Our runner will record all these intermediate results to avoid missing the optimal result. Furthermore, we have implemented an \textit{Early-Stop Strategy} heuristic. This strategy operates on a sliding-window approach, where it examines $T$ consecutive results to detect any signs of improvement. If a consistent trend of improvement is observed within the window, the algorithm moves on to the next set of results without interruption. However, if a result within the current window is worse than the best result identified across all prior recorded, this is taken as an indication of a local minimum. Upon recognizing such a local minimum, the \textit{Early-Stop Strategy} triggers a termination control signal to the runner, causing the rewriting process to halt early. In contrast to the previous approach of setting termination conditions quantitatively, Our runner in runtime mode with \textit{Early-Stop Strategy}  not only saves significant runtime during the rewriting and extraction processes but also ensures the preservation of the optimal solution.

%\textbf{Runner in quality mode :} In quality mode, we opt for a different approach. Instead of frequent intervals, we select a set of fixed check points that are spaced further apart, such as at iterations [ 3, 30, 60 ,90]. This strategy is deliberately designed to explore solutions that are distributed across various regions of the solution space, aiming to uncover a broader spectrum of potential optima. At each check point, regarding the extraction cost function, we employ a tunable tree-based cost function that enables randomness. This is modulated by a probability factor $K$ ranging from 0 to 0.3, which allows $eclasses$ to select some of some $enodes$ with suboptimal costs.This process generates $N$ groups of samplings through random extraction in parallel, complemented by 1 solution obtained from DAG-based extraction. This approach significantly increases the variation in the solution space, allowing for greater exploration of different possibilities.  

% \guangyu{I recommend to rename the faster-bottom up  with a totally different name. like fluctuating-based-extraction}







% We build an interface, utilizing Rust's serde library, that connects the rewriting runner in the egg framework to a new extraction library - extraction gym ,which effectively addresses the third problem mentioned in section II B.Bottom-up extraction algorithm works by 
% iteratively computing the current best cost of each node in the e-graph based on the current best costs of its children.Extraction terminates when our estimates of the best cost for each node reach a fixed point.Faster Bottom-up extraction algorithm instead uses fxhashmap, compared to the standard HashMap,which demonstrates better performance on large e-graphs.what's more,it only visits the nodes whose current cost estimate may change:it does this by tracking parent-child relationships and storing relevant nodes in a work list (UniqueQueue).

% \subsubsection{random and dag based cost function}







% \cchen{faster random simulation}


% \subsection{Integration with the Existing Synthesis Flow}\label{sec:integrate}

% % \begin{figure*}[tbp]  
% %     \centering
% %     \begin{minipage}{0.49\textwidth}
% %         \centering
% %         \includegraphics[width=\textwidth]{figs/conv_flow_comp.pdf}
% %         \caption{Cp}
% %     \end{minipage}
% %      \label{fig:}
% %     \hfill 
% %     \begin{minipage}{0.49\textwidth}
% %         \centering
% %         \includegraphics[width=\textwidth]{figs/conv_operator_comp.pdf}
% %         \caption{Ours}
% %     \end{minipage}
% %     \vspace{-1em}
% %     \caption{} 
% %     \label{fig:}
% % \end{figure*}


% \guangyu{add a flow chart to this part}
% The DAG-aware multi-level optimization operator based on the And Inverter Graph (AIG) in \texttt{ABC} generally adheres to a common design principle: It iteratively traverses every node in the AIG and performs a cut enumeration for each node to identify its corresponding 4-input or 5-input subgraph. Subsequently, it replaces the subgraph with a lower-cost but functionally equivalent one that has already been precomputed. When this type of operators are invoked multiple times and fails to find a lower-cost subgraph that can be replaced, it is very likely to converge to a local optimum, which limits the solution space explored. Below, we will illustrate two ways in which \deftextEsynTurbo  can assist ABC in mitigating this issue.

% \deftextEsynTurbo can be utilized as a standalone operator: a semi-global and non-destructive  rewriting operator configured in a delay/area-oriented mode, which offers competitive speed and quality of results (QoR) optimization performance compared to operators within ABC, with specific experiments detailed in Section 4.3. By adjusting the number of rewriting rounds and the random probability parameter, \deftextEsynTurbo can identify a large set of equivalent representations, serving as a highly flexible new operator that can be seamlessly integrated with many existing sequence of operations  exploration work that leveraging machine learning and reinforcement learning, such as FlowTune~\cite{flowtune},Alphasyn~\cite{alphasyn} to expand the solution space of similar works.

% \deftextEsynTurbo can also be integrated into the existing ABC optimization flow: Typically, these flows first perform a series of technology-independent optimizations to reduce the AIG to a smaller logic level and the number of AND gates, then apply the \texttt{dch} operator:  \texttt{dch} command combines different networks observed during technology-independent synthesis into a single network with choices. This aids the subsequent technology mapping to better select the logic structure with optimal costs. Finally, technology mapping is conducted based on the given technology library. We will integrate \deftextEsynTurbo  after the technology-independent optimizations, using this converged local optimum after technology-independent optimizations as the starting point. By combining \deftextEsynTurbo with a random sampling approach, we can help escape the local optimum, covering the surrounding solution space. This provides a variety of initial state candidates before applying \texttt{dch} , which is more conducive to finding a solution with better PPA characteristics.



==> figs/pareto_compare.tex <==
\begin{figure*}
    \centering
        \begin{minipage}{.3\textwidth}
            \begin{subfigure}{\textwidth}
            \centering
            \includegraphics[width=\textwidth]{figs/EPFL_adder_pareto.pdf}
            \caption{adder}
            \end{subfigure}\\
            \begin{subfigure}{\textwidth}
            \centering
            \includegraphics[width=\textwidth]{example-image-b}
            \caption{}
            \end{subfigure}%    
            \caption{Small Size Circuit}
        \end{minipage}
        \hfill
        \begin{minipage}{.3\textwidth}
            \begin{subfigure}{\textwidth}
            \centering
            \includegraphics[width=\textwidth]{figs/EPFL_multiplier_pareto.pdf}
            \caption{multiplier}
            \end{subfigure}\\
            \begin{subfigure}{\textwidth}
            \centering
            \includegraphics[width=\textwidth]{example-image-b}
            \caption{}
            \end{subfigure}%    
            \caption{Medium Size Circuit}
        \end{minipage}
        \hfill
        \begin{minipage}{.3\textwidth}
            \begin{subfigure}{\textwidth}
            \centering
            \includegraphics[width=\textwidth]{example-image-a}
            \caption{}
            \end{subfigure}\\
            \begin{subfigure}{\textwidth}
            \centering
            \includegraphics[width=\textwidth]{example-image-b}
            \caption{}
            \end{subfigure}%    
            \caption{Large Size Circuit}
        \end{minipage}%
        \caption{Pareto Frontier Comparison on EPFL Benchmark}
\end{figure*}

==> figs/scalability_comp.tex <==
\begin{tikzpicture}
\begin{axis}[
    ybar,
    enlargelimits=0.15,
    legend style={at={(0.5,-0.25)},
      anchor=north, legend columns=-1},
    ylabel={Normalized Value},
    symbolic x coords={DAC23, ASILOMAR23, ASPLOS24, DAC24, EsynTurbo},
    xtick=data,
    xticklabels={
    \tiny{DAC'23~\cite{coward2023automating}}, \tiny{ASILOMAR23'\cite{Wanna2023MultiplierOV}}, \tiny{ASPLOS'24~\cite{cheng2023seer}}, \tiny{DAC'24\cite{chen2024syn}}, 
    \tiny{\textbf{Ours}}
    },
    xticklabel style={rotate=-45, anchor=north west}, % Rotates labels and adjusts anchor
   % nodes near coords,
    nodes near coords align={vertical},
    title={Comparative Analysis of Circuit Size \\for Maximum-Mentioned Circuit},
    title style={align=center}
]
\addplot 
  coordinates {(DAC23,0.0021) (ASILOMAR23,0.000037) 
    (ASPLOS24,0.0021) (DAC24,0.0111) (EsynTurbo,1.0)};
\addplot 
  coordinates {(DAC23,0.0008) (ASILOMAR23,0.00026) 
    (ASPLOS24,0.0008) (DAC24,0.0061) (EsynTurbo,1.0)};
\legend{Level, Size}
\end{axis}
\end{tikzpicture}

% DAC'23 - https://arxiv.org/pdf/2303.01839.pdf
% circuit with largest area: interpolation, 433 um^2
% circuit with longest delay: FP Sub, 285 ps

% ASILOMAR'23 - https://arxiv.org/pdf/2312.06004.pdf
% circuit with largest area:  6-bit squarer, 7.9 um^2
% circuit with longest delay: 8 bit multiplier, 93.6 ps

% ASPLOS'24 (SEER) - https://arxiv.org/pdf/2308.07654.pdf
% circuit with largest area: grid, 132 um^2
% circuit with longest delay: byte_enable_calc, 976 ps

% DAC'24 (Esyn) - https://arxiv.org/pdf/2403.14242v2.pdf
% circuit with largest area:  bar, 2338 um^2
% circuit with longest delay: adder, 2173 ps

% Ours
% circuit with largest area:  hyp, 211076 um^2
% circuit with longest delay:  hyp, 354592 ps

==> sections/Thoughs.tex <==
\guangyu{

- Maybe I can mention the largest graph we can cover (sell the scalability). Like, how many e-nodes we can handle, how large circuit we can handle.

}

==> tables/DSE_random_setting.tex <==
% \begin{table}[H]
% \centering
% \caption{The Random Parameter For Design Space Exploration.}
% \label{tab:dse_iter} 
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{c||c|c|c}
% \hline 
% Phase& Hyper-Parameter&\textit{w.} Random& \textit{w.o.} Random \\
% \hline \hline 
% Rewrite& \#.Iteration&$[3,30,60,90]$& Determined by \textit{Early-Stop}\\
% \hline
% \multirow{3}{*}{Extract} & Extractor Type&$[$Tree-based, DAG-based$]$& Tree-based \\
% \cline{2-4}
% & Random Probability& $[0,0.1,0.2,0.3]$& 0 \\
% \cline{2-4}
% & Cost Function& [Size, Depth]& Depth\\
% \cline{2-4}
% & \#.Extract Circuit & 20 & 1 \\
% \hline
% \multirow{2}{*}{Fuzzing} & \#. Fuzzing Passes & 400 & 500 \\
% \cline{2-4}
% & Length of Passes & 15-20 & 15-20 \\
% \hline
% \end{tabular}}
% \end{table}

% \begin{table}[H]
% \centering
% \caption{The parameter for design space exploration. We randomly selected 400 circuits generated by different hyper-parameter in \deftextEsynTurbo, comparing ABC's hyper-volumn by optimization passes fuzzing.}
% \label{tab:dse_iter} 
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{c||c|c|c}
% \hline 
% Phase& Hyper-Parameter&\deftextEsynTurbo \textit{w.} Tuning& ABC\\
% \hline \hline 
% Rewrite& \#.~Iteration&$[3,30,60,90]$& -\\
% \hline
% \multirow{3}{*}{Extract} & Extractor Type&$[$\textit{Tree}-based, \textit{DAG}-based$]$& -\\
% \cline{2-4}
% & Random Probability& $[0,0.1,0.2,0.3]$& -\\
% \cline{2-4}
% & Cost Function& $[Size, Depth]$& -\\
% \cline{2-4}
% & \#. Extract Circuit& 20 & - \\
% \hline
% \multirow{2}{*}{Opt. Fuzzing} 
% & \#. Fuzzing Passes per Circuit & 20 & 500 \\
% \cline{2-4}
% & \#. Fuzzing Passes in Total & $\textcolor{teal}{400}~(20~Cric *20~Passes)$ & $500~(1~Circ *500~Passes)$\\
% \cline{2-4}
% & Length of Passes & \textcolor{teal}{10-15} & 15-20 \\
% \hline
% \end{tabular}}

% % \begin{tablenotes}
% % \item $^\star$ There is only one circuit to test different passes.
% % \end{tablenotes}
% \label{table:dse-tuning}
% \end{table}

\begin{table}[!b]
\centering
\caption{The parameters for quality-oriented mode and the setting for operator fuzzing in design space exploration. }
%We randomly selected 400 circuits generated by different hyper-parameter in \deftextEsynTurbo, comparing ABC's hypervolume by optimization operators fuzzing.
\label{tab:dse_iter2} 
\resizebox{\columnwidth}{!}{
\begin{tabular}{c||c|c|c}
\hline 
Phase& Hyper-Parameter&\deftextEsynTurbo \textit{w.} Tuning& ABC\\
\hline \hline 
Rewrite& \#.~Iteration&$[3,30,60,90]$& -\\
\hline
\multirow{3}{*}{Extract} & Extractor Type&$[$\textit{Tree}-based, \textit{DAG}-based$]$& -\\
\cline{2-4}
& Random Probability& $[0,0.1,0.2,0.3]$& -\\
\cline{2-4}
& Cost Function& $[Size, Depth]$& -\\
\cline{2-4}
& \#. Extract Circuit& 1-400 & - \\
\hline
\multirow{2}{*}{Opt. Fuzzing} 
% & \#. Fuzzing Passes per Circuit & 20 & 500 \\
% \cline{2-4}
& \#. Fuzzing Operators in Total & $\textcolor{teal}{400}$ & $500~(1~Circ *500~Passes)$\\
\cline{2-4}
& Length of Operators & \textcolor{teal}{10-15} & 15-20 \\
\hline
\end{tabular}}

% \begin{tablenotes}
% \item $^\star$ There is only one circuit to test different passes.
% \end{tablenotes}
\label{table:dse-tuning}
\end{table}

==> tables/compare_with_epfl_best_res.tex <==
\begin{table*}
\centering
\caption{Comparing the technology mapping results with EPFL best depth optimization circuits}
\label{early_stop} 
\resizebox{0.8\columnwidth}{!}{
\begin{tabular}{|l|c|c|c|c|}
\hline
\multirow{2}{*}{\textbf{Design}} & \multicolumn{2}{c|}{\textbf{EPFL Best Depth Result}} & \multicolumn{2}{c|}{\textbf{Optimized \textit{w.} \deftextEsynTurbo}} \\ \cline{2-5} 
 & \textbf{Delay ($ps$)} & \textbf{Area ($um^2$)} & \textbf{Delay ($ps$)} & \textbf{Area ($um^2$)} 

 \\ \hline
adder  
 % iter 30 + st;dch -f;st;timing;timing;read_lib asap7_clean.lib;map;topo;upsize;dnsize;stime
& 382.93&         1751.00& \textbf{248.70}& 2739.87\\ \hline
bar             
% iter 20 + st;dch -f;st;timing;timing;read_lib asap7_clean.lib;map;topo;upsize;dnsize;stime
& 209.74&       2320.67& 281.37& \textbf{2263.52} 
\\ \hline
 div& 44199.00& 121543.55& 59070.66&154383.06\\

\hline

 hyp & 623836.25& 805446.31& &\\

 \hline

  log2& 5218.23& 47886.0& &\\

  \hline

  max & 758.38& 3474.01& &\\

  \hline

  multiplier 
  %iter 80 + st;dch -f;st;timing;timing;read_lib asap7_clean.lib;map;topo;upsize;dnsize;stime
  & 2511.88 & 56612.39& 2913.69& \textbf{38251.62}\\

  \hline

  sin & 57541.57& 2694534.00& &\\

  \hline

  sqrt & 152817.73& 131647.38& &\\

  \hline

  square & 764.50& 31334.40& &\\

  \hline

  arbiter %iter 60 + st;dch -f;st;timing;timing;read_lib asap7_clean.lib;map;topo;upsize;dnsize;stime
  & 389.16 & 1420.91 & \textbf{259.94} & 4289.55 \\

  \hline

  cavlc & 215.72& 845.17& &\\

  \hline

  ctrl & 82.72& 111.97& &\\

  \hline

  dec & 77.07& 428.77& &\\

  \hline

  i2c & 269.65& 895.33& &\\

  \hline

  int2float & 163.99& 300.93& &\\

  \hline

  mem\_ctrl & 403.87& 7092.65& &\\

  \hline

  priority & 194.81& 501.32& &\\

  \hline

  router & 135.33& 121.54& &\\

  \hline

  voter & 897.29& 21508.18& &\\

  \hline

\end{tabular}}
\end{table*}




==> tables/design_sapce_exploration_table.tex <==
\begin{table*}[h]
\centering
\caption{DSE}
\label{tab} 
\cchen{voter  hyp}
\resizebox{\linewidth}{!}{%
\begin{tabular}{|l|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{\textbf{Design}} & \multicolumn{3}{c|}{\textbf{ABC$\_$random$\_$fuzz2000}\cite{}} & \multicolumn{3}{c|}{\textbf{Ours}} \\ \cline{2-7} 
 & \textbf{Area-oriented($\mu m^2$)} & \textbf{Delay-oriented($ps$)} & \textbf{ADP-oriented} & \textbf{Area-oriented($\mu m^2$)} & \textbf{Delay-oriented($ps$)} & \textbf{ADP-oriented} \\ \hline
adder              & 843           & 2313           & \textbf{2631003}           & \textbf{839}  & \textbf{644}           & \textbf{1248072}         \\ \hline
bar                & 2230          & 230          & \textbf{587088}           & \textbf{2203}     & \textbf{193}           & \textbf{438397}      \\ \hline
div                & 23073             & 55770              &  1297265970          & \textbf{23621}       & \textbf{61717}           & \textbf{1436371812}   \\ \hline
hyp                &            &             & \textbf{}                &  \textbf{}             & \textbf{}           & \textbf{}  \\ \hline
log2               & 25988              & 4342             & 118003734          & \textbf{27781}        & \textbf{4405}           & \textbf{126653579}  \\ \hline
max                & 2278              & 1687              & 3934084          & \textbf{2350}        & \textbf{1583}           & \textbf{3937940}   \\ \hline
multiplier         & 20318            & 3188             & 69640960         & \textbf{21452}       & \textbf{2791}           & \textbf{62124992}   \\ \hline
sin                & 5274              & 2498             & 13344316           & \textbf{5646}       & \textbf{2611}           & \textbf{15001422}    \\ \hline
sqrt               &  16508             &  66567             & 1275623421           & \textbf{}      & \textbf{}           & \textbf{}    \\ \hline
square             &    14765           &   2034            & 32145336          & \textbf{}     & \textbf{}           & \textbf{}      \\ \hline
arbiter            &  7773          & 726          & \textbf{6144864}           & \textbf{6705}    & \textbf{900}           & \textbf{6041205}       \\ \hline
cavlc              & 455           & 106          & \textbf{53192}           & \textbf{475}     & \textbf{97}           & \textbf{50925}      \\ \hline
ctrl               & 78           & 46           & 4263           &       &          &    \\ \hline
dec                & 351          & 69          & \textbf{24219}           & \textbf{351}   & \textbf{53}           & \textbf{24219}        \\ \hline
i2c                & 744            & 110           & \textbf{93830}           & 834     & \textbf{103}           & \textbf{94348}    \\ \hline
int2float          & 144           & 70           & \textbf{11704}           & 156      & \textbf{71}           & \textbf{12136}    \\ \hline
mem\_ctrl           & 26177              & 1237              & \textbf{33801050}          & \textbf{29306}    & \textbf{1318}           & \textbf{38771606}      \\ \hline
priority           & 359              & 548              & 214323          & \textbf{666}       & \textbf{1389}           & \textbf{1290380}    \\ \hline
router             & 116           & 128          & 16000 & 146    & \textbf{152}           & \textbf{22192}       \\ \hline
voter              &             &               & \textbf{}           & \textbf{}        & \textbf{}           & \textbf{}   \\ \hline
\end{tabular}}
\end{table*}

==> tables/early_stop_130nm.tex <==
\begin{table*}[h]
\centering
% \caption{Comparing the different technology-independent optimization sequence with Esynturbo using \textit{Early-Stop} Strategy with the following command in ABC~\cite{} :
% \textit{\textbf{ strash; map; topo; upsize; dnsize; stime}}. The delay of these are obtained after technology mapping using the ASAP 7nm ~\cite{}predictive standard-cell library. \cchen{{WIP Update ours result in EsynTurb}}} ~\
\caption{Comparing delay-oriented operators in ABC, including dc2, resyn2, and dch with \deftextEsynTurbo. The delay results are obtained after technology mapping using the SkyWater 130 nm PDK library. }
\label{} 
\resizebox{\linewidth}{!}{
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{\textbf{Design}} &  \multicolumn{3}{|c|}{\textbf{\textit{dch}}} &  \multicolumn{3}{c|}{\textbf{\textit{resyn2}}} & \multicolumn{3}{|c|}{\textbf{\textit{dc2}}} & \multicolumn{3}{c|}{\textbf{\deftextEsynTurbo w \textit{Early-Stop}}}& \multicolumn{3}{c|}{\textbf{\deftextEsynTurbo w/o \textit{Early-Stop }}} \\ \cline{2-16}

&\textbf{lev} & \textbf{Delay($ps$)} & \textbf{runtime($s$)}&\textbf{lev} & \textbf{Delay($ps$)} & \textbf{runtime($s$)}&\textbf{lev} & \textbf{Delay($ps$)} & \textbf{runtime($s$)} &\textbf{lev}& \textbf{Delay($ps$)} & \textbf{runtime($s$)} &\textbf{lev}& \textbf{Delay($ps$)} & \textbf{runtime($s$)}\\ \hline
     cavlc & 13 & 728.95 & 0.3 & 16 & 846.49 & 0.31 & 17 & 837.63 & 0.6 & ~ & ~ & ~ & 12 & 717.98 & 386.95 \\ \hline
        int2float & 10 & 518.61 & 0.22 & 15 & 690.76 & 0.26 & 13 & 581.22 & 0.22 & ~ & ~ & ~ & 9 & 527.28 & 458.85 \\ \hline
        sqrt & 4969 & 460257.12 & 14.59 & 4968 & 518289.25 & 13.75 & 6065 & 390184.28 & 16.64 & ~ & ~ & ~ & 4997 & 499437.75 & 360.81 \\ \hline
        dec & 3 & 402.39 & 0.23 & 3 & 402.39 & 0.3 & 3 & 402.39 & 0.25 & ~ & ~ & ~ & 3 & 404.36 & 28.8 \\ \hline
        square & 248 & 15182.22 & 3.2 & 248 & 15078.76 & 3.9 & 248 & 15273.2 & 2.99 & ~ & ~ & ~ & 212 & 12307.89 & 552.87 \\ \hline
        multiplier & 262 & 17361.96 & 6.59 & 262 & 17560.43 & 6.43 & 262 & 17530.65 & 5.75 & ~ & ~ & ~ & 250 & 24175.43 & 620.51 \\ \hline
        voter & 55 & 4332.19 & 3.94 & 57 & 4538.17 & 2.81 & 59 & 4415.2 & 2.18 & ~ & ~ & ~ & 68 & 5583.31 & 1314.15 \\ \hline
        priority & 202 & 12428.5 & 0.51 & 203 & 11507.33 & 0.42 & 216 & 13069.15 & 0.46 & ~ & ~ & ~ & 126 & 7948.02 & 324.46 \\ \hline
        arbiter & 87 & 4339.93 & 8.21 & 87 & 4983.6 & 3.96 & 89 & 4629.53 & 4.82 & ~ & ~ & ~ & 45 & 2430.89 & 386 \\ \hline
        adder & 255 & 15328.44 & 0.73 & 255 & 13988.86 & 0.62 & 255 & 15022.15 & 0.54 & ~ & ~ & ~ & 68 & 4232.48 & 333.18 \\ \hline
        mem\_ctrl & 91 & 7635.35 & 14.62 & 110 & 8908.52 & 7.58 & 98 & 8569.68 & 7.24 & ~ & ~ & ~ & 103 & 10056.55 & 347.75 \\ \hline
        hyp & 24689 & 2409397.75 & 1112.14 & 24794 & 2071158.25 & 174.07 & 24873 & 1831879.12 & 135.43 & ~ & ~ & ~ & 20783 & 1999075.88 & 543.55 \\ \hline
        max & 163 & 11391.95 & 0.66 & 200 & 12089.89 & 0.73 & 213 & 13826.68 & 0.9 & ~ & ~ & ~ & 152 & 10338.64 & 365.44 \\ \hline
        router & 23 & 1313.1 & 0.25 & 19 & 1130.89 & 0.58 & 26 & 1426.21 & 0.43 & ~ & ~ & ~ & 30 & 1455.82 & 372.68 \\ \hline
        div & 4375 & 319761.81 & 13.93 & 4361 & 327621 & 10.55 & 4397 & 316733.59 & 11.88 & ~ & ~ & ~ & 4343 & 331610.72 & 390.3 \\ \hline
        log2 & 362 & 24411.71 & 13.28 & 376 & 26340.08 & 9.2 & 358 & 25561.53 & 8.64 & ~ & ~ & ~ & 395 & 28119.88 & 326.6 \\ \hline
        i2c & 14 & 918.09 & 0.36 & 15 & 881.87 & 0.33 & 14 & 1041.29 & 0.34 & ~ & ~ & ~ & 12 & 721.96 & 401.86 \\ \hline
        bar & 12 & 1414.86 & 0.69 & 12 & 1495.41 & 0.61 & 14 & 1498.7 & 0.63 & ~ & ~ & ~ & 11 & 2894.12 & 496.82 \\ \hline
        sin & 158 & 13010.84 & 2.21 & 177 & 13746.03 & 1.76 & 161 & 12836.06 & 1.71 & ~ & ~ & ~ & 169 & 13557.76 & 334.12 \\ \hline
\end{tabular}}
\end{table*}



% \begin{table*}[h]
% \centering
% \caption{Comparing the different technology-independent optimization sequence with Esynturbo using \textit{Early-Stop} Strategy with the following command in ABC~\cite{} :
% \textit{\textbf{ strash; map; topo; upsize; dnsize; stime}}. The delay of these are obtained after technology mapping using the SkyWater 130 nm PDK~\cite{}predictive standard-cell library. \cchen{{WIP Update ours result in EsynTurb}}} ~\

% \label{early_stop} 
% \resizebox{\linewidth}{!}{
% \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
% \hline
% \multirow{2}{*}{\textbf{Design}} &  \multicolumn{3}{|c|}{\textbf{\textit{dch}}} &  \multicolumn{3}{c|}{\textbf{\textit{resyn2}}} & \multicolumn{3}{|c|}{\textbf{\textit{dc2}}} & \multicolumn{3}{c|}{\textbf{\deftextEsynTurbo w. \textit{Early-Stop}}}& \multicolumn{3}{c|}{\textbf{\deftextEsynTurbo w. \textit{Early-Stop } + dch}}& \multicolumn{3}{c|}{\textbf{\deftextEsynTurbo w. \textit{Early-Stop} + dc2}} \\ \cline{2-19}

% &\textbf{lev} & \textbf{Delay($ps$)} & \textbf{runtime($s$)}&\textbf{lev} & \textbf{Delay($ps$)} & \textbf{runtime($s$)}&\textbf{lev} & \textbf{Delay($ps$)} & \textbf{runtime($s$)} &\textbf{lev}& \textbf{Delay($ps$)} & \textbf{runtime($s$)} &\textbf{lev}& \textbf{Delay($ps$)} & \textbf{runtime($s$)} &\textbf{lev} & \textbf{Delay($ps$)} & \textbf{runtime($s$)}\\ \hline
%   cavlc & 13 & 728.95 & 0.35 & 16 & 846.49 & 0.34 & 17 & 837.63 & 0.33 & 14 & 775.27 & 0.67 & 13 & 686.09 & 0.7 & 16 & 846.67 & 0.66 \\ \hline
%         int2float & 10 & 518.61 & 0.26 & 15 & 690.76 & 0.32 & 13 & 581.22 & 0.26 & 12 & 602.38 & 0.44 & 10 & 585.04 & 0.44 & 11 & 489.19 & 0.43 \\ \hline
%         sqrt & 4969 & 460257.12 & 12.02 & 4968 & 518289.25 & 12.78 & 6065 & 390184.28 & 14.11 & 5057 & 486174.06 & 23.75 & 4977 & 458235.06 & 14.13 & 6057 & 458801.66 & 17.52 \\ \hline
%         dec & 3 & 402.39 & 0.27 & 3 & 402.39 & 0.3 & 3 & 402.39 & 0.27 & 3 & 370.33 & 0.39 & 3 & 402.39 & 0.39 & 3 & 402.39 & 0.4 \\ \hline
%         square & 248 & 15182.22 & 3.09 & 248 & 15078.76 & 3.01 & 248 & 15273.2 & 2.29 & 249 & 16532.59 & 5.6 & 247 & 14828.19 & 5.67 & 247 & 15130.04 & 4.9 \\ \hline
%         multiplier & 262 & 17361.96 & 5.51 & 262 & 17560.43 & 5.88 & 262 & 17530.65 & 5.06 & 274 & 18772.88 & 8.01 & 262 & 17209.74 & 11.0 & 262 & 17122.9 & 10.64 \\ \hline
%         voter & 55 & 4332.19 & 3.69 & 57 & 4538.17 & 2.7 & 59 & 4415.2 & 1.99 & 70 & 5400.65 & 4.03 & 57 & 4196.77 & 5.57 & 63 & 4410.81 & 3.75 \\ \hline
%         priority & 202 & 12428.5 & 0.57 & 203 & 11507.33 & 0.49 & 216 & 13069.15 & 0.43 & 250 & 15358.57 & 0.99 & 203 & 12530.36 & 0.69 & 216 & 13069.1 & 0.66 \\ \hline
%         arbiter & 87 & 4339.93 & 6.99 & 87 & 4983.6 & 3.89 & 89 & 4629.53 & 4.38 & 87 & 4870.13 & 6.29 & 87 & 4438.73 & 9.86 & 88 & 4980.54 & 5.14 \\ \hline
%         adder & 255 & 15328.44 & 0.69 & 255 & 13988.86 & 0.62 & 255 & 15022.15 & 0.3 & 193 & 8648.72 & 0.79 & 193 & 8243.77 & 0.75 & 255 & 13169.61 & 0.72 \\ \hline
%         mem\_ctrl & 91 & 7635.35 & 11.93 & 110 & 8908.52 & 5.72 & 98 & 8569.68 & 6.08 & 114 & 9599.41 & 10.07 & 89 & 8271.11 & 18.01 & 96 & 8279.15 & 11.61 \\ \hline
%         hyp & 24689 & 2409397.75 & 786.7 & 24794 & 2071158.25 & 148.33 & 24873 & 1831879.12 & 116.61 & 24801 & 1782300.25 & 249.48 & 24673 & 2407694.25 & 904.19 & 24879 & 1787475.38 & 152.12 \\ \hline
%         max & 163 & 11391.95 & 0.78 & 200 & 12089.89 & 0.8 & 213 & 13826.68 & 1.0 & 231 & 14778.4 & 1.47 & 148 & 10527.65 & 1.25 & 209 & 13732.29 & 1.31 \\ \hline
%         router & 23 & 1313.1 & 0.27 & 19 & 1130.89 & 0.25 & 26 & 1426.21 & 0.21 & 30 & 1625.51 & 0.49 & 20 & 1110.36 & 0.42 & 25 & 1210.72 & 0.47 \\ \hline
%         div & 4375 & 319761.81 & 12.42 & 4361 & 327621.0 & 9.56 & 4397 & 316733.59 & 11.17 & 4372 & 334109.97 & 22.17 & 4377 & 322364.44 & 19.85 & 4409 & 315761.47 & 21.22 \\ \hline
%         log2 & 362 & 24411.71 & 12.0 & 376 & 26340.08 & 8.4 & 358 & 25561.53 & 7.56 & 444 & 28182.71 & 10.15 & 332 & 23015.79 & 16.89 & 358 & 25241.66 & 11.47 \\ \hline
%         i2c & 14 & 918.09 & 0.43 & 15 & 881.87 & 0.4 & 14 & 1041.29 & 0.4 & 15 & 848.23 & 0.67 & 12 & 854.54 & 0.86 & 14 & 844.88 & 0.72 \\ \hline
%         ctrl & 7 & 332.2 & 0.23 & 8 & 378.17 & 0.26 & 7 & 337.98 & 0.24 & 7 & 342.35 & 0.39 & 6 & 399.19 & 0.4 & 8 & 370.78 & 0.39 \\ \hline
%         bar & 12 & 1414.86 & 0.73 & 12 & 1495.41 & 0.73 & 14 & 1498.7 & 0.68 & 12 & 1670.46 & 1.12 & 12 & 1438.88 & 1.24 & 14 & 1515.13 & 1.14 \\ \hline
%         sin & 158 & 13010.84 & 2.37 & 177 & 13746.03 & 1.83 & 161 & 12836.06 & 1.59 & 215 & 13886.14 & 2.43 & 158 & 12831.37 & 2.86 & 160 & 13136.18 & 2.25 \\ \hline
% \end{tabular}}
% \end{table*}


==> tables/early_stop_45nm.tex <==

\begin{table*}[h]
\centering
% \caption{Comparing the different technology-independent optimization sequence with Esynturbo using \textit{Early-Stop} Strategy with the following command in ABC~\cite{} :
% \textit{\textbf{ strash; map; topo; upsize; dnsize; stime}}. The delay of these are obtained after technology mapping using the ASAP 7nm ~\cite{}predictive standard-cell library. \cchen{{WIP Update ours result in EsynTurb}}} ~\
\caption{Comparing delay-oriented operators in ABC, including dc2, resyn2, and dch with \deftextEsynTurbo. The delay results are obtained after technology mapping using the FreePDK45\textsuperscript{TM} 45nm library. }
\label{early_stop} 
\resizebox{\linewidth}{!}{
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{\textbf{Design}} &  \multicolumn{3}{|c|}{\textbf{\textit{dch}}} &  \multicolumn{3}{c|}{\textbf{\textit{resyn2}}} & \multicolumn{3}{|c|}{\textbf{\textit{dc2}}} & \multicolumn{3}{c|}{\textbf{\deftextEsynTurbo w \textit{Early-Stop}}}& \multicolumn{3}{c|}{\textbf{\deftextEsynTurbo w/o \textit{Early-Stop }}} \\ \cline{2-16}

&\textbf{lev} & \textbf{Delay($ps$)} & \textbf{runtime($s$)}&\textbf{lev} & \textbf{Delay($ps$)} & \textbf{runtime($s$)}&\textbf{lev} & \textbf{Delay($ps$)} & \textbf{runtime($s$)} &\textbf{lev}& \textbf{Delay($ps$)} & \textbf{runtime($s$)} &\textbf{lev}& \textbf{Delay($ps$)} & \textbf{runtime($s$)}\\ \hline
     cavlc & 13 & 728.95 & 0.3 & 16 & 846.49 & 0.31 & 17 & 837.63 & 0.6 & ~ & ~ & ~ & 12 & 717.98 & 386.95 \\ \hline
        int2float & 10 & 518.61 & 0.22 & 15 & 690.76 & 0.26 & 13 & 581.22 & 0.22 & ~ & ~ & ~ & 9 & 527.28 & 458.85 \\ \hline
        sqrt & 4969 & 460257.12 & 14.59 & 4968 & 518289.25 & 13.75 & 6065 & 390184.28 & 16.64 & ~ & ~ & ~ & 4997 & 499437.75 & 360.81 \\ \hline
        dec & 3 & 402.39 & 0.23 & 3 & 402.39 & 0.3 & 3 & 402.39 & 0.25 & ~ & ~ & ~ & 3 & 404.36 & 28.8 \\ \hline
        square & 248 & 15182.22 & 3.2 & 248 & 15078.76 & 3.9 & 248 & 15273.2 & 2.99 & ~ & ~ & ~ & 212 & 12307.89 & 552.87 \\ \hline
        multiplier & 262 & 17361.96 & 6.59 & 262 & 17560.43 & 6.43 & 262 & 17530.65 & 5.75 & ~ & ~ & ~ & 250 & 24175.43 & 620.51 \\ \hline
        voter & 55 & 4332.19 & 3.94 & 57 & 4538.17 & 2.81 & 59 & 4415.2 & 2.18 & ~ & ~ & ~ & 68 & 5583.31 & 1314.15 \\ \hline
        priority & 202 & 12428.5 & 0.51 & 203 & 11507.33 & 0.42 & 216 & 13069.15 & 0.46 & ~ & ~ & ~ & 126 & 7948.02 & 324.46 \\ \hline
        arbiter & 87 & 4339.93 & 8.21 & 87 & 4983.6 & 3.96 & 89 & 4629.53 & 4.82 & ~ & ~ & ~ & 45 & 2430.89 & 386 \\ \hline
        adder & 255 & 15328.44 & 0.73 & 255 & 13988.86 & 0.62 & 255 & 15022.15 & 0.54 & ~ & ~ & ~ & 68 & 4232.48 & 333.18 \\ \hline
        mem\_ctrl & 91 & 7635.35 & 14.62 & 110 & 8908.52 & 7.58 & 98 & 8569.68 & 7.24 & ~ & ~ & ~ & 103 & 10056.55 & 347.75 \\ \hline
        hyp & 24689 & 2409397.75 & 1112.14 & 24794 & 2071158.25 & 174.07 & 24873 & 1831879.12 & 135.43 & ~ & ~ & ~ & 20783 & 1999075.88 & 543.55 \\ \hline
        max & 163 & 11391.95 & 0.66 & 200 & 12089.89 & 0.73 & 213 & 13826.68 & 0.9 & ~ & ~ & ~ & 152 & 10338.64 & 365.44 \\ \hline
        router & 23 & 1313.1 & 0.25 & 19 & 1130.89 & 0.58 & 26 & 1426.21 & 0.43 & ~ & ~ & ~ & 30 & 1455.82 & 372.68 \\ \hline
        div & 4375 & 319761.81 & 13.93 & 4361 & 327621 & 10.55 & 4397 & 316733.59 & 11.88 & ~ & ~ & ~ & 4343 & 331610.72 & 390.3 \\ \hline
        log2 & 362 & 24411.71 & 13.28 & 376 & 26340.08 & 9.2 & 358 & 25561.53 & 8.64 & ~ & ~ & ~ & 395 & 28119.88 & 326.6 \\ \hline
        i2c & 14 & 918.09 & 0.36 & 15 & 881.87 & 0.33 & 14 & 1041.29 & 0.34 & ~ & ~ & ~ & 12 & 721.96 & 401.86 \\ \hline
        bar & 12 & 1414.86 & 0.69 & 12 & 1495.41 & 0.61 & 14 & 1498.7 & 0.63 & ~ & ~ & ~ & 11 & 2894.12 & 496.82 \\ \hline
        sin & 158 & 13010.84 & 2.21 & 177 & 13746.03 & 1.76 & 161 & 12836.06 & 1.71 & ~ & ~ & ~ & 169 & 13557.76 & 334.12 \\ \hline
\end{tabular}}
\end{table*}


% \begin{table*}[h]
% \centering
% \caption{Comparing the different technology-independent optimization sequence with Esynturbo using \textit{Early-Stop} Strategy with the following command in ABC~\cite{} :
% \textit{\textbf{ strash; map; topo; upsize; dnsize; stime}}. The delay of these are obtained after technology mapping using the FreePDK45\textsuperscript{TM} 45nm~\cite{}predictive standard-cell library. \cchen{{WIP Update ours result in EsynTurb}}} ~\

% \label{early_stop} 
% \resizebox{0.8\linewidth}{!}{
% \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|}
% \hline
% \multirow{2}{*}{\textbf{Design}} &  \multicolumn{3}{|c|}{\textbf{\textit{dch}}} &  \multicolumn{3}{c|}{\textbf{\textit{resyn2}}} & \multicolumn{3}{|c|}{\textbf{\textit{dc2}}} & \multicolumn{3}{c|}{\textbf{\deftextEsynTurbo w. \textit{Early-Stop}}} \\ \cline{2-13}

% &\textbf{lev} & \textbf{Delay($ps$)} & \textbf{runtime($s$)} &\textbf{lev}& \textbf{Delay($ps$)} & \textbf{runtime($s$)} &\textbf{lev}& \textbf{Delay($ps$)} & \textbf{runtime($s$)} &\textbf{lev} & \textbf{Delay($ps$)} & \textbf{runtime($s$)}\\ \hline
%         cavlc & 13 & 172.92 & 0.237699519 & 16 & 193.62 & 0.271235047 & 17 & 217.27 & 0.21138639 & 14 & 181.18 & 0.46550382 \\ \hline
%         int2float & 10 & 166.35 & 0.156773013 & 15 & 166.26 & 0.19212402 & 13 & 151.56 & 0.150802824 & 12 & 141.51 & 0.316386735 \\ \hline
%         sqrt & 4969 & 106824.12 & 10.591415373 & 4968 & 104861.77 & 7.736188798 & 6065 & 104611.52 & 4.887667927 & 5057 & 114329.55 & 10.921864659 \\ \hline
%         dec & 3 & 79.61 & 0.181401751 & 3 & 79.61 & 0.2138787 & 3 & 79.61 & 0.176311635 & 3 & 79.61 & 0.292824626 \\ \hline
%         square & 248 & 3309.72 & 2.47142009 & 248 & 3327.95 & 2.353204045 & 248 & 3132.16 & 1.691225743 & 249 & 3328.01 & 4.169194485 \\ \hline
%         multiplier & 262 & 3818.87 & 7.62108828 & 262 & 3934.32 & 5.382808867 & 262 & 3960.34 & 5.271906738 & 274 & 3969.14 & 6.960882116 \\ \hline
%         voter & 55 & 1026.68 & 3.395467263 & 57 & 1065.71 & 2.002225547 & 59 & 1048.41 & 1.829709623 & 70 & 1312.72 & 4.130378429 \\ \hline
%         priority & 202 & 2926.76 & 0.268804226 & 203 & 2618.91 & 0.435875386 & 216 & 3129.22 & 0.287377904 & 250 & 3590.58 & 0.499753511 \\ \hline
%         arbiter & 87 & 1097.81 & 4.383181129 & 87 & 1097.81 & 1.818722071 & 89 & 1088.27 & 2.634392707 & 87 & 1079.38 & 3.902345181 \\ \hline
%         adder & 255 & 3104.05 & 0.309143681 & 255 & 3092.34 & 0.372282839 & 255 & 3283.42 & 0.285392376 & 193 & 2740.65 & 0.626202793 \\ \hline
%         mem\_ctrl & 91 & 1753.26 & 10.113500785 & 110 & 2040.74 & 3.979169896 & 98 & 1780.23 & 4.11759103 & 114 & 2233.3 & 7.889600145 \\ \hline
%         hyp & 24689 & 445831.88 & 773.967846834 & 24794 & 416708.75 & 75.275022007 & 24873 & 436958.0 & 35.252189266 & 24801 & 406735.06 & 76.753164064 \\ \hline
%         max & 163 & 2639.74 & 0.563214441 & 200 & 3022.97 & 0.752723191 & 213 & 3228.42 & 0.507965944 & 231 & 3692.62 & 1.093229817 \\ \hline
%         router & 23 & 355.19 & 0.165133918 & 19 & 259.91 & 0.194472953 & 26 & 335.38 & 0.164767881 & 30 & 410.04 & 0.384858582 \\ \hline
%         div & 4375 & 66698.94 & 10.42489127 & 4361 & 67168.03 & 12.418370708 & 4397 & 67350.72 & 6.012291619 & 4372 & 70652.59 & 15.521644184 \\ \hline
%         log2 & 362 & 5816.79 & 9.770663469 & 376 & 6073.02 & 5.767934381 & 358 & 6144.54 & 4.769453292 & 444 & 6549.17 & 7.656859676 \\ \hline
%         i2c & 14 & 204.24 & 0.258081992 & 15 & 234.0 & 0.24534141 & 14 & 197.68 & 0.21780231 & 15 & 206.27 & 0.506945306 \\ \hline
%         ctrl & 7 & 84.86 & 0.140204954 & 8 & 103.37 & 0.169111351 & 7 & 87.87 & 0.147742489 & 7 & 92.16 & 0.291260547 \\ \hline
%         bar & 12 & 461.91 & 0.485381625 & 12 & 550.46 & 0.649892446 & 14 & 464.23 & 0.453365054 & 12 & 478.52 & 0.834536073 \\ \hline
%         sin & 158 & 3047.39 & 2.085325089 & 177 & 3213.45 & 1.214335848 & 161 & 3030.11 & 1.322592518 & 215 & 3356.85 & 1.966800819 \\ \hline
% \end{tabular}}
% \end{table*}



==> tables/early_stop_7nm.tex <==


\begin{table*}[h]
\centering
\caption{Comparing delay-oriented operators in ABC, including dc2, resyn2, and dch with \deftextEsynTurbo. The delay results are obtained after technology mapping using the ASAP 7nm library. }
\label{earlystop} 
\resizebox{\linewidth}{!}{
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{\textbf{Design}} &  \multicolumn{3}{|c|}{\textbf{\textit{dch}}} &  \multicolumn{3}{c|}{\textbf{\textit{resyn2}}} & \multicolumn{3}{|c|}{\textbf{\textit{dc2}}} & \multicolumn{3}{c|}{\textbf{\deftextEsynTurbo w \textit{Early-Stop}}}& \multicolumn{3}{c|}{\textbf{\deftextEsynTurbo w/o \textit{Early-Stop }}} \\ \cline{2-16}

&\textbf{lev} & \textbf{Delay($ps$)} & \textbf{runtime($s$)}&\textbf{lev} & \textbf{Delay($ps$)} & \textbf{runtime($s$)}&\textbf{lev} & \textbf{Delay($ps$)} & \textbf{runtime($s$)} &\textbf{lev}& \textbf{Delay($ps$)} & \textbf{runtime($s$)} &\textbf{lev}& \textbf{Delay($ps$)} & \textbf{runtime($s$)}\\ \hline
  cavlc & 13 & 120.55 & 0.75 & 16 & 126.31 & 0.73 & 17 & 128.3 & 0.71 & 14 & \textbf{120.01} & 3.47 & 12 & 104.99 & 347.23 \\ \hline
        int2float & 10 & 79.18 & 0.64 & 15 & 101.39 & 0.65 & 13 & 101.89 & 0.64 & 10 & \textbf{74.38} & 2.41 & 9 & 89.5 & 436.07 \\ \hline
        sqrt & 4969 & 106864.79 & 9.54 & 4968 & 100931.82 & 8.79 & 6065 & 81114.03 & 4.51 & 5057 & \textbf{87412.19} & 24.06 & 4997 & 92698.32 & 337.99 \\ \hline
        dec & 3 & 69.63 & 0.67 & 3 & 69.63 & 0.69 & 3 & 69.63 & 0.67 & 4 & \textbf{68.65} & 1.99 & 3 & 61.11 & 19.73 \\ \hline
        square & 248 & 3014.28 & 3.13 & 248 & 2418.47 & 3.01 & 248 & 3042.11 & 2.17 & 249 & \textbf{2393.16} & 7.5 & 212 & 2047.49 & 508.32 \\ \hline
        multiplier & 262 & 3293.72 & 4.58 & 262 & 3351.4 & 5.03 & 262 & 3315.69 & 3.79 & 260 & \textbf{3084.94} & 15.64 & 250 & 3153.45 & 484.7 \\ \hline
        voter & 55 & 850.29 & 3.29 & 57 & 863.22 & 2.82 & 59 & 818.28 & 1.77 & 70 & 1025 & 3.29 & 68 & 1148.8 & 320.05 \\ \hline
        priority & 202 & 1930.24 & 0.65 & 203 & 1932.05 & 0.72 & 216 & 2121.13 & 0.7 & 250 & \textbf{2094.23} & 3.33 & 126 & 1224.61 & 323.74 \\ \hline
        arbiter & 87 & 951.68 & 8.7 & 87 & 728.51 & 5.4 & 89 & 849.17 & 3.41 & 87 & \textbf{727.95} & 8.7 & 45 & 443.61 & 441.17 \\ \hline
        adder & 255 & 2901.95 & 0.87 & 255 & 2757.96 & 0.63 & 255 & 2723.03 & 0.76 & 192 & \textbf{1655.36} & 3.14 & 68 & 677.68 & 320.55 \\ \hline
        mem\_ctrl & 91 & 1642.43 & 11.4 & 110 & 1806.44 & 5.23 & 98 & 1604.31 & 5.22 & 114 & 1744.66 & 14.32 & 103 & 2959.42 & 321.17 \\ \hline
        hyp & 24689 & 357287.09 & 440.71 & 24794 & 361072.16 & 99.31 & 24873 & 470401.34 & 59.49 & 24801 & \textbf{352762.50} & 133.86 & 20783 & 373686.72 & 449.11 \\ \hline
        max & 163 & 1907.32 & 0.87 & 200 & 2216.41 & 1.02 & 213 & 2798.07 & 1.07 & 253 & 2488.61 & 6.3 & 152 & 1768.76 & 325.53 \\ \hline
        router & 23 & 228.37 & 0.65 & 19 & 177.28 & 0.67 & 26 & 282.13 & 0.54 & 30 & 258.59 & 2.37 & 30 & 270.32 & 376.99 \\ \hline
        div & 4375 & 67410.44 & 14.43 & 4361 & 66309.74 & 10.02 & 4397 & 69860.64 & 8.01 & 4372 & \textbf{51098.14} & 37.5 & 4343 & 51742.13 & 373.82 \\ \hline
        log2 & 362 & 4794.31 & 10.46 & 376 & 4664.04 & 9.82 & 358 & 4540.24 & 7.09 & 444 & 5228.17 & 18.37 & 395 & 5880.52 & 322.17 \\ \hline
        i2c & 14 & 172.99 & 0.78 & 15 & 137.57 & 0.63 & 14 & 242.62 & 0.74 & 14 & \textbf{107.83} & 3.90 & 12 & 189.85 & 430.13 \\ \hline
        ctrl & 7 & 67.03 & 0.65 & 7 & 49.44 & 0.63 & 7 & 49.83 & 0.63 & 7 & 58.25 & 1.86 & 6 & 59.57 & 89.3 \\ \hline
        bar & 12 & 243.64 & 0.97 & 12 & 281.5 & 0.99 & 14 & 291.88 & 0.78 & 13 & 272.37 & 3.57 & 11 & 269.12 & 416.64 \\ \hline
        sin & 158 & 2705.22 & 2.52 & 177 & 2667.49 & 1.79 & 161 & 2643.51 & 1.66 & 216 & 2799.76 & 4.33 & 169 & 3004.56 & 329.81 \\ \hline
        Avg & 1799.9 & 27826.7575 & 25.813 & 1809.25 & 27633.1415 & 7.929 & 1869.4 & 32349.8915 & 5.218 & 1822.85 & 25773.7375 & 14.9955 & 1589.7 & 27074.0265 & 348.711 \\ \hline
        Impr. [\%] &~& \color{green!50!black}{7} & \color{green!50!black}{42} &~& \color{green!50!black}{7} & \color{red}{-89} & ~&\color{green!50!black}{20} & \color{red}{-187} & ~ & ~ & ~ & ~& \color{green!50!black}{5} & \color{green!50!black}{96}   \\ 
        \hline
\end{tabular}}
\end{table*}







==> tables/esynturbo_refine_operator_130nm.tex <==


\begin{table*}[h]
\centering
\caption{Comparing delay-oriented operators in ABC, including dc2, resyn2, and dch with \deftextEsynTurbo. The delay results are obtained after technology mapping using the SkyWater 130 nm PDK library. }

\label{refine130} 
\resizebox{\linewidth}{!}{
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{\textbf{Design}} &  \multicolumn{5}{|c|}{\textbf{\textit{dc2}}} &  \multicolumn{5}{c|}{\textbf{\deftextEsynTurbo w. \textit{Early-Stop } + dc2}} & \multicolumn{5}{|c|}{\textbf{\textit{dch}}} & \multicolumn{5}{c|}{\textbf{\deftextEsynTurbo w. \textit{Early-Stop} + dch}}\\ \cline{2-21}

&\textbf{and}&\textbf{Area ($\mu m^2$)} &\textbf{lev} & \textbf{Delay($ps$)} & \textbf{runtime($s$)}&\textbf{and}&\textbf{Area ($\mu m^2$)}&\textbf{lev} & \textbf{Delay($ps$)} & \textbf{runtime($s$)}&\textbf{and}&\textbf{Area ($\mu m^2$)}&\textbf{lev} & \textbf{Delay($ps$)} & \textbf{runtime($s$)} &\textbf{and}&\textbf{Area ($\mu m^2$)}&\textbf{lev}& \textbf{Delay($ps$)} & \textbf{runtime($s$)} \\ \hline
        cavlc & 649 & 2319.72 & 17 & 837.63 & 0.33 & 639 & 2309.72 & 15 & 732.2 & 3.62 & 639 & 2282.19 & 13 & 728.95 & 0.35 & 634 & 2319.72 & 12 & 685.26 & 3.76 \\ \hline
        int2float & 208 & 800.77 & 13 & 581.22 & 0.26 & 202 & 788.26 & 11 & 489.19 & 1.48 & 207 & 731.95 & 10 & 518.61 & 0.26 & 208 & 769.49 & 10 & 495.47 & 3.84 \\ \hline
        sqrt & 18452 & 90505.55 & 6065 & 390184.28 & 14.11 & 18465 & 85450.7 & 6057 & 458801.66 & 19.79 & 19326 & 110313.3 & 4969 & 460257.12 & 12.02 & 19328 & 108250.07 & 4977 & 458235.06 & 26.48 \\ \hline
        dec & 304 & 1705.39 & 3 & 402.39 & 0.27 & 304 & 1705.39 & 3 & 402.39 & 1.12 & 304 & 1705.39 & 3 & 402.39 & 0.27 & 304 & 1705.39 & 3 & 402.39 & 2.42 \\ \hline
        square & 16676 & 66532.56 & 248 & 15273.2 & 2.29 & 17156 & 69337.75 & 247 & 13728.49 & 12.04 & 16640 & 67123.12 & 248 & 15182.22 & 3.09 & 17159 & 69867.01 & 220 & 12147.18 & 13.7 \\ \hline
        multiplier & 24377 & 94844.71 & 262 & 17530.65 & 5.06 & 24379 & 95835.66 & 262 & 17122.9 & 16.83 & 24579 & 97922.66 & 262 & 17361.96 & 5.51 & 24582 & 99645.56 & 262 & 17216.68 & 18.48 \\ \hline
        voter & 8597 & 51719.6 & 59 & 4415.2 & 1.99 & 8625 & 49824.04 & 63 & 4410.81 & 5.66 & 8583 & 52694.29 & 55 & 4332.19 & 3.69 & 8574 & 50368.30 & 57 & 4196.77 & 5.75 \\ \hline
        priority & 703 & 3218.09 & 216 & 13069.15 & 0.43 & 1316 & 5438.97 & 190 & 9782.79 & 3.45 & 670 & 3687.29 & 202 & 12428.5 & 0.57 & 851 & 3789.88 & 149 & 8982.54 & 3.17 \\ \hline
        arbiter & 11839 & 43286.52 & 89 & 4629.53 & 4.38 & 11839 & 42131.66 & 89 & 4765.27 & 9.03 & 11840 & 44581.51 & 87 & 4339.93 & 6.99 & 11857 & 42386.9 & 87 & 4435 & 11.12 \\ \hline
        adder & 1019 & 4858.41 & 255 & 15022.15 & 0.3 & 1254 & 5938.2 & 214 & 10006.76 & 3.21 & 1019 & 6902.87 & 255 & 15328.44 & 0.69 & 1266 & 6104.6 & 193 & 8243.77 & 2.11 \\ \hline
        mem\_ctrl & 42755 & 132345.67 & 98 & 8569.68 & 6.08 & 42831 & 132330.66 & 96 & 8279.15 & 14.81 & 41728 & 129651.84 & 91 & 7635.35 & 11.93 & 41933 & 130088.52 & 93 & 7714.58 & 36.74 \\ \hline
        hyp & 211688 & 920570.38 & 24873 & 1831879.12 & 116.61 & 212744 & 973378.5 & 24878 & 1791684.50 & 188.22 & 211694 & 892318.31 & 24689 & 2409397.75 & 786.7 & 212674 & 1036197.50 & 24687 & 2243522.25 & 717.47 \\ \hline
        max & 2833 & 11019.32 & 213 & 13826.68 & 1 & 2860 & 10645.21 & 182 & 11817.88 & 4.022 & 2831 & 10023.36 & 163 & 11391.95 & 0.78 & 2837 & 10188.52 & 148 & 10527.65 & 1.92 \\ \hline
        router & 223 & 1103.56 & 26 & 1426.21 & 0.21 & 186 & 782 & 22 & 1092.91 & 2.20 & 201 & 980.94 & 23 & 1313.1 & 0.27 & 175 & 744.46 & 19 & 1022.69 & 3.975 \\ \hline
        div & 40443 & 188454.48 & 4397 & 316733.59 & 11.17 & 40433 & 192225.61 & 4404 & 315253.06 & 30.95 & 30808 & 137819.67 & 4375 & 319761.81 & 12.42 & 30796 & 142655.56 & 4374 & 319666.91 & 29.11 \\ \hline
        log2 & 29323 & 112223.88 & 358 & 25561.53 & 7.56 & 29318 & 115001.55 & 358 & 24979.49 & 19.01 & 29039 & 121204.99 & 362 & 24411.71 & 12 & 28767 & 119931.27 & 305 & 23086.99 & 27.74 \\ \hline
        i2c & 1136 & 3827.42 & 14 & 1041.29 & 0.4 & 1128 & 4096.43 & 14 & 772.06 & 1.93 & 1095 & 3723.57 & 14 & 918.09 & 0.43 & 1089 & 3816.16 & 11 & 789.4 & 1.78 \\ \hline
        ctrl & 96 & 419.15 & 7 & 337.98 & 0.24 & 103 & 501.73 & 7 & 312.9 & 1.44 & 91 & 427.91 & 7 & 332.2 & 0.23 & 110 & 474.2 & 6 & 362.24 & 1.31 \\ \hline
        bar & 2952 & 10747.81 & 14 & 1498.7 & 0.68 & 2957 & 10780.34 & 14 & 1488.6 & 4.1 & 2952 & 10651.47 & 12 & 1414.86 & 0.73 & 2952 & 10438.76 & 12 & 1421.45 & 3.61 \\ \hline
        sin & 5040 & 24450.95 & 161 & 12836.06 & 1.59 & 5071 & 24274.53 & 162 & 12747.33 & 4.7 & 5023 & 25126.6 & 158 & 13010.84 & 2.37 & 5047 & 24482.23 & 158 & 12811.74 & 4.85 \\ \hline
        geomean & 3712.18 & 15708.13 & 119.53 & 8076.21 & 1.54 & 3849.72 & 16186.32 & 114.43 & 7366.15 & 6.33 & 3616.55 & 15849.55 & 110.74 & 7853.79 & 2.09 & 3714.91 & 15780.17 & 102.34 & 7170.83 & 7.78 \\ \hline
        Impr. [\%] ~ & ~ & ~ & ~ & ~ & ~& \color{red}{-4} & \color{red}{-3} & \color{green!50!black}{4} & \color{green!50!black}{9} & ~&  &~  & ~ & ~ & ~ & \color{red}{-3} & 0 & \color{green!50!black}{8} & \color{green!50!black}{9}& ~\\ \hline
        

\end{tabular}}
\end{table*}



% \begin{table*}[h]
% \centering
% \caption{Comparing the different technology-independent optimization sequence with Esynturbo using \textit{Early-Stop} Strategy with the following command in ABC~\cite{} :
% \textit{\textbf{ strash; map; topo; upsize; dnsize; stime}}. The delay of these are obtained after technology mapping using the FreePDK45\textsuperscript{TM} 45nm~\cite{}predictive standard-cell library. \cchen{{WIP Update ours result in EsynTurb}}} ~\

% \label{early_stop} 
% \resizebox{0.8\linewidth}{!}{
% \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|}
% \hline
% \multirow{2}{*}{\textbf{Design}} &  \multicolumn{3}{|c|}{\textbf{\textit{dch}}} &  \multicolumn{3}{c|}{\textbf{\textit{resyn2}}} & \multicolumn{3}{|c|}{\textbf{\textit{dc2}}} & \multicolumn{3}{c|}{\textbf{\deftextEsynTurbo w. \textit{Early-Stop}}} \\ \cline{2-13}

% &\textbf{lev} & \textbf{Delay($ps$)} & \textbf{runtime($s$)} &\textbf{lev}& \textbf{Delay($ps$)} & \textbf{runtime($s$)} &\textbf{lev}& \textbf{Delay($ps$)} & \textbf{runtime($s$)} &\textbf{lev} & \textbf{Delay($ps$)} & \textbf{runtime($s$)}\\ \hline
%         cavlc & 13 & 172.92 & 0.237699519 & 16 & 193.62 & 0.271235047 & 17 & 217.27 & 0.21138639 & 14 & 181.18 & 0.46550382 \\ \hline
%         int2float & 10 & 166.35 & 0.156773013 & 15 & 166.26 & 0.19212402 & 13 & 151.56 & 0.150802824 & 12 & 141.51 & 0.316386735 \\ \hline
%         sqrt & 4969 & 106824.12 & 10.591415373 & 4968 & 104861.77 & 7.736188798 & 6065 & 104611.52 & 4.887667927 & 5057 & 114329.55 & 10.921864659 \\ \hline
%         dec & 3 & 79.61 & 0.181401751 & 3 & 79.61 & 0.2138787 & 3 & 79.61 & 0.176311635 & 3 & 79.61 & 0.292824626 \\ \hline
%         square & 248 & 3309.72 & 2.47142009 & 248 & 3327.95 & 2.353204045 & 248 & 3132.16 & 1.691225743 & 249 & 3328.01 & 4.169194485 \\ \hline
%         multiplier & 262 & 3818.87 & 7.62108828 & 262 & 3934.32 & 5.382808867 & 262 & 3960.34 & 5.271906738 & 274 & 3969.14 & 6.960882116 \\ \hline
%         voter & 55 & 1026.68 & 3.395467263 & 57 & 1065.71 & 2.002225547 & 59 & 1048.41 & 1.829709623 & 70 & 1312.72 & 4.130378429 \\ \hline
%         priority & 202 & 2926.76 & 0.268804226 & 203 & 2618.91 & 0.435875386 & 216 & 3129.22 & 0.287377904 & 250 & 3590.58 & 0.499753511 \\ \hline
%         arbiter & 87 & 1097.81 & 4.383181129 & 87 & 1097.81 & 1.818722071 & 89 & 1088.27 & 2.634392707 & 87 & 1079.38 & 3.902345181 \\ \hline
%         adder & 255 & 3104.05 & 0.309143681 & 255 & 3092.34 & 0.372282839 & 255 & 3283.42 & 0.285392376 & 193 & 2740.65 & 0.626202793 \\ \hline
%         mem\_ctrl & 91 & 1753.26 & 10.113500785 & 110 & 2040.74 & 3.979169896 & 98 & 1780.23 & 4.11759103 & 114 & 2233.3 & 7.889600145 \\ \hline
%         hyp & 24689 & 445831.88 & 773.967846834 & 24794 & 416708.75 & 75.275022007 & 24873 & 436958.0 & 35.252189266 & 24801 & 406735.06 & 76.753164064 \\ \hline
%         max & 163 & 2639.74 & 0.563214441 & 200 & 3022.97 & 0.752723191 & 213 & 3228.42 & 0.507965944 & 231 & 3692.62 & 1.093229817 \\ \hline
%         router & 23 & 355.19 & 0.165133918 & 19 & 259.91 & 0.194472953 & 26 & 335.38 & 0.164767881 & 30 & 410.04 & 0.384858582 \\ \hline
%         div & 4375 & 66698.94 & 10.42489127 & 4361 & 67168.03 & 12.418370708 & 4397 & 67350.72 & 6.012291619 & 4372 & 70652.59 & 15.521644184 \\ \hline
%         log2 & 362 & 5816.79 & 9.770663469 & 376 & 6073.02 & 5.767934381 & 358 & 6144.54 & 4.769453292 & 444 & 6549.17 & 7.656859676 \\ \hline
%         i2c & 14 & 204.24 & 0.258081992 & 15 & 234.0 & 0.24534141 & 14 & 197.68 & 0.21780231 & 15 & 206.27 & 0.506945306 \\ \hline
%         ctrl & 7 & 84.86 & 0.140204954 & 8 & 103.37 & 0.169111351 & 7 & 87.87 & 0.147742489 & 7 & 92.16 & 0.291260547 \\ \hline
%         bar & 12 & 461.91 & 0.485381625 & 12 & 550.46 & 0.649892446 & 14 & 464.23 & 0.453365054 & 12 & 478.52 & 0.834536073 \\ \hline
%         sin & 158 & 3047.39 & 2.085325089 & 177 & 3213.45 & 1.214335848 & 161 & 3030.11 & 1.322592518 & 215 & 3356.85 & 1.966800819 \\ \hline
% \end{tabular}}
% \end{table*}



==> tables/esynturbo_refine_operator_7nm.tex <==


\begin{table*}[h]
\centering
\caption{Comparing delay-oriented operators in ABC, including dc2, resyn2, and dch with \deftextEsynTurbo. The delay results are obtained after technology mapping using the ASAP 7nm library. }

\label{refine7} 
\resizebox{\linewidth}{!}{
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{\textbf{Design}} &  \multicolumn{5}{|c|}{\textbf{\textit{dc2}}} &  \multicolumn{5}{c|}{\textbf{\deftextEsynTurbo w. \textit{Early-Stop } + dc2}} & \multicolumn{5}{|c|}{\textbf{\textit{dch}}} & \multicolumn{5}{c|}{\textbf{\deftextEsynTurbo w. \textit{Early-Stop} + dch}}\\ \cline{2-21}

&\textbf{and}&\textbf{Area ($\mu m^2$)} &\textbf{lev} & \textbf{Delay($ps$)} & \textbf{runtime($s$)}&\textbf{and}&\textbf{Area ($\mu m^2$)}&\textbf{lev} & \textbf{Delay($ps$)} & \textbf{runtime($s$)}&\textbf{and}&\textbf{Area ($\mu m^2$)}&\textbf{lev} & \textbf{Delay($ps$)} & \textbf{runtime($s$)} &\textbf{and}&\textbf{Area ($\mu m^2$)}&\textbf{lev}& \textbf{Delay($ps$)} & \textbf{runtime($s$)} \\ \hline
cavlc & 649 & 475.19 & 17 & 128.3 & 0.62 & \textbf{645} & 481.49 & \textbf{15} & \textbf{116.23} & 7.58 & 639 & 489.65 & 13 & 120.55 & 0.9 & \textbf{638} & 493.62 & 15 & \textbf{108.45} & 3.61 \\ \hline
int2float & 208 & 153.5 & 13 & 101.89 & 0.66 &\textbf{ 202} & 172.16 & \textbf{11} & \textbf{77.12} & 3.9 & 207 & 170.99 & 10 & 79.18 & 0.72 & 207 & \textbf{162.83} & 10 & 80.39 & 6.29 \\ \hline
sqrt & 18452 & 19753.22 & 6065 & 81114.03 & 4.57 & 18464 & 19856.33 & 6068 & \textbf{79232.68} & 17.79 & 19326 & 24172.71 & 4969 & 106864.79 & 9.93 & 19328 & \textbf{24041.6} & 4977 & \textbf{97659.4} & 22.8 \\ \hline
dec & 304 & 351.55 & 3 & 69.63 & 0.86 & 304 & 351.55 & 3 & 69.63 & 5.3 & 304 & 351.55 & 3 & 69.63 & 0.81 & 304 & 351.55 & 3 & 69.63 & 5.17 \\ \hline
square & 16676 & 15679.45 & 248 & 3042.11 & 2.13 & 16902 & 16082.32 & \textbf{247} & \textbf{2174.21} & 11.18 & 16640 & 15925.79 & 248 & 3014.28 & 3.28 & 17022 & \textbf{15730.54} & \textbf{247} & \textbf{3003.68} & 15.82 \\ \hline
multiplier & 24377 & 21977.31 & 262 & 3315.69 & 4.72 & \textbf{24375} & 22240.91 & 262 & \textbf{3280.22 }& 17.72 & 24579 & 22475.13 & 262 & 3293.72 & 5.4 & 24588 & \textbf{22339.59} & 262 & \textbf{3273.48} & 27.83 \\ \hline
voter & 8597 & 11681.96 & 59 & 818.28 & 1.83 & 8630 & \textbf{11562.29} & 62 & 825.32 & 16.72 & 8583 & 12473.01 & 55 & 850.29 & 3.41 & 8574 & \textbf{11879.32} & 57 & \textbf{828.41 }& 11.9 \\ \hline
priority & 703 & 791.05 & 216 & 2121.13 & 0.61 & 734 & 1006.6 & \textbf{215} &\textbf{ 1969.8 }& 8.11 & 670 & 639.65 & 202 & 1930.24 & 0.67 & 851 & 919.12 & \textbf{149} & \textbf{1718.55 }& 7.86 \\ \hline
arbiter & 11839 & 7758.19 & 89 & 849.17 & 4.25 & 11839 & \textbf{7679.58} & \textbf{88} & 945.84 & 8.7 & 11840 & 7893.03 & 87 & 951.68 & 9.28 &\textbf{ 11311} & \textbf{7312.16} & 87 &\textbf{ 941.07} & 17.76 \\ \hline
adder & 1019 & 1157.07 & 255 & 2723.03 & 0.82 & 1254 & 1255.75 & \textbf{214} & \textbf{1921.73} & 7.18 & 1019 & 1258.55 & 255 & 2901.95 & 0.83 & 1335 & 1391.52 & \textbf{133} & \textbf{1049.99} & 7.8 \\ \hline
mem\_ctrl & 42755 & 29303 & 98 & 1604.31 & 5.52 & 42831 & 29397.25 & \textbf{96} & \textbf{1546.27} & 26.1 & 41728 & 28652.85 & 91 & 1642.43 & 12.59 & 42005 & 29004.87 & \textbf{89} & \textbf{1512.89} & 29.11 \\ \hline
hyp & 211688 & 212334.25 & 24873 & 470401.34 & 71.8 & 212742 & 222647.8 & 24874 & 489135.41 & 208.571 & 211694 & 203284.62 & 24689 & 357287.09 & 1026.52 & 212696 & 208010.64 & \textbf{24685 }& 365492 & 1118.53 \\ \hline
max & 2833 & 2420.98 & 213 & 2798.07 & 0.91 & 2833 & 2542.99 & \textbf{206 }& \textbf{2179.61} & 5.93 & 2831 & 2510.79 & 163 & 1907.32 & 0.89 & 2833 & \textbf{2386.92} & \textbf{158} & \textbf{1756.25} & 5.79 \\ \hline
router & 223 & 218.58 & 26 & 282.13 & 0.64 & \textbf{185} & \textbf{146.73} & \textbf{23 }&\textbf{ 205.33} & 4.29 & 201 & 202.49 & 23 & 228.37 & 0.6 & 209 & \textbf{199.92} & \textbf{19} & \textbf{162.05} & 4.58 \\ \hline
div & 40443 & 47284.22 & 4397 & 69860.64 & 9.04 & \textbf{40431 }& \textbf{46605.61} & 4409 & \textbf{66474.01 }& 29.92 & 30808 & 34323.19 & 4375 & 67410.44 & 16.92 & 30978 & \textbf{34307.09} & 4377 & \textbf{64754.64} & 44.85 \\ \hline
log2 & 29323 & 26513.44 & 358 & 4540.24 & 9.23 & \textbf{29320 }& 26856.83 & 359 & \textbf{4511.33 }& 38.77 & 29039 & 28396.24 & 362 & 4794.31 & 12.59 & \textbf{28787 }& 29376.25 & \textbf{330} & \textbf{4568.78} & 44.24 \\ \hline
i2c & 1136 & 819.75 & 14 & 242.62 & 0.85 & \textbf{1131 }& 846.34 & 14 & \textbf{145.73} & 4.93 & 1095 & 808.32 & 14 & 172.99 & 0.77 & 1111 & 873.4 & \textbf{12} & \textbf{126.13} & 5.6 \\ \hline
ctrl & 96 & 100.31 & 7 & 49.83 & 0.56 & 110 & \textbf{95.18} & \textbf{6 }& \textbf{46.03} & 1.86 & 91 & 96.11 & 7 & 48.29 & 0.98 & 115 & 109.87 & \textbf{6 }& \textbf{45.62} & 3.168 \\ \hline
bar & 2952 & 2302.47 & 14 & 291.88 & 1.22 & 2952 & 2305.51 & 14 & \textbf{284.21} & 6.52 & 2952 & 2416.31 & 12 & 243.64 & 1.17 & 2952 & \textbf{2410.72} & 12 & \textbf{236.68 }& 6.16 \\ \hline
sin & 5040 & 5873.52 & 161 & 2643.51 & 1.67 & 5051 & \textbf{5735.19} & 162 & 2691.62 & 7.59 & 5023 & 6027.96 & 158 & 2705.22 & 3.08 & 5061 & \textbf{5863.26 }& 160 & \textbf{2695.16 }& 16.64 \\ \hline
GEOMEAN & 3712.18 & 3476.39 & 119.53 & 1534.92 & 2.01 & 3746.96 & 3498.94 & 115.1 & 1370.04 & 10.63 & 3616.55 & 3474.97 & 110.74 & 1439.21 & 3.09 & 3761.9 & 3555.74 & 103.19 & 1280.34 & 13.61 \\ \hline
Impr. [\%] ~ & ~ & ~ & ~ & ~ & ~& \color{red}{-1} & \color{red}{-1} & \color{green!50!black}{4} & \color{green!50!black}{11}  & ~ & ~ & ~ & ~ & ~ & ~ & \color{red}{-4} & \color{red}{-2} & \color{green!50!black}{7} & \color{green!50!black}{11} & ~\\ \hline
        % Impr.  & ~ & ~ & ~ & ~ & ~ & -1\% & -1\% & 4\% & 11\% & ~ & ~ & ~ & ~ & ~ & ~ & -4\% & -2\% & 7\% & 11\% & ~ \\ \hline
\end{tabular}}
\end{table*}


==> tables/extraction_time_table.tex <==
\begin{table}[h]
\centering
\caption{Extraction time comparision. Which consume the most of time of optimization.}
\resizebox{0.7\columnwidth}{!}{
\begin{tabular}{|c|c|c|}
\hline
\textbf{Design} & \textbf{Vanilla extractor  ($s$)} & \textbf{Ours}  ($s$) \\
\hline
adder & 2.92 & 0.36 \\ \hline
arbiter & 3.30 & 0.71 \\ \hline
bar & 1.23 & 0.53 \\ \hline
cavlc & 0.55 & 0.36 \\ \hline
ctrl & 0.28 & 0.16 \\ \hline
dec & 3.17 & 0.26 \\ \hline
div & 1005.99 & 3.5 \\ \hline
hyp &  &  \\ \hline
i2c & 1.57 & 0.74 \\ \hline
int2float & 0.50 & 0.36 \\ \hline
log2 & 27.95 & 2.21 \\ \hline
max & 5.21 & 0.49 \\ \hline
mem\_ctrl & 229.51 & 2.99 \\ \hline
multiplier & 30.74 & 2.9 \\ \hline
priority & 7.43 & 0.57 \\ \hline
router & 0.76 & 0.18 \\ \hline
sin & 2.82 & 0.35 \\ \hline
sqrt & 93.60 & 1.19 \\ \hline
square & 26.84 & 2.42 \\ \hline
voter & 3.46 &  \\ \hline
\end{tabular}
}
\end{table}

==> tables/hyper_volumn_comp.tex <==
\centering
\vspace{4ex}
\resizebox{\linewidth}{!}{
\begin{NiceTabular}{cc|c|c|c|c|c|c}
\RowStyle[bold]{}
Design & adder & max & square & arbiter & multiplier & mem\_ctrl & Averaged \\
\hline 
Arbitrary Fuzz &  0.31& 0.84 &  0.91 & 0.64  & 0.62  & 0.97 & 0.715 \\
\hline 
\deftextEsynTurbo & $\textbf{1.000}$ & $\textbf{1.000}$ & $\textbf{1.000}$ & $\textbf{1.000}$ & $\textbf{1.000}$ & $\textbf{1.000}$ & $\textbf{1.000}$ \\
\CodeAfter
  \OverBrace[yshift=1mm,shorten]{1-2}{1-3}{\text{Small circuit}}
  \OverBrace[yshift=1mm,shorten]{1-4}{1-5}{\text{Medium circuit}}
  \OverBrace[yshift=1mm,shorten]{1-6}{1-7}{\text{Large circuit}}
\end{NiceTabular}}
\label{table:hv_comp}

==> tables/operator_comp.tex <==

\begin{table}
\caption{Comparison of AIG Statistics, ABC if, and Ours (if -g -K 6 -C 8)\guangyu{add the additional fig on the rhs?}}
\centering
\small
\setlength{\tabcolsep}{4pt}
%if -g -K 6  -C 8
%if -g
\resizebox{0.95\columnwidth}{!}{
\begin{tabular}{l|rrr|rrr|}
\hline
\multirow{2}{*}{\textbf{Benchmarks}} & \multicolumn{3}{c|}{\textbf{ABC} \texttt{if -g}} 
& \multicolumn{3}{c|}{\textbf{Ours}}  \\
&Area ($\mu m^2$)&Delay ($ps$)&Time ($s$)&Area ($\mu m^2$)&Delay ($ps$)&Time ($s$)\\
\hline
  adder & 1274.41 & 943.3 & 1.17 & 2066.86 & 659.11 & 16.20  \\ \hline
        max & 2746.87 & 1614.2 & 1.24 & 2729.61 & 1663.94 & 7.33  \\ \hline
        square & 17165.44 & 1093.99 & 4.06 & 21687.34 & 1930.33 & 13.38  \\ \hline
        %arbiter & 5636.51 & 282.95 & 2.4 & 8457.33 & 727.95 & 6.85  \\ \hline
        sqrt & 48189.35 & 101509.26 & 29.28 & 23122.01 & 87456.66 & 14.93  \\ \hline
        log2 & 39170.51 & 6311.65 & 10.6 & 25969.9 & 5228.17 & 12.12  \\ \hline
        div & 74448.98 & 35435.32 & 24.54 & 63367.01 & 48799.02 & 26.01  \\ \hline
        hyp & 294667.41 & 382960.22 & 145.44 & 200680.28 & 347414.25 & 96.15  \\ \hline
        multiplier & 33125.29 & 3083.43 & 5.79 & 25069.9 & 3350.99 & 8.94  \\ \hline
        mem\_ctrl & 37079.39 & 1897.24 & 6.88 & 32422.19 & 1744.66 & 14.06  \\ \hline
        %AVG & 55350.416 & 53513.156 & 23.093 & 40487.096 & 50030.355 & 19.952  \\ \hline
        Impr & ~& ~ & ~ & \textbf{26.9\%} & \textbf{6.5\%} & \textbf{13.6\%}  \\ \hline
\hline
\end{tabular}}
\label{tab:comparison}
\end{table}


% rs (if -g)}
% \centering
% \small
% \setlength{\tabcolsep}{4pt}
% %if -g -K 6  -C 8
% %if -g
% \resizebox{0.95\columnwidth}{!}{
% \begin{tabular}{l|rrr|rrr|}
% \hline
% \multirow{2}{*}{\textbf{Benchmarks}} & \multicolumn{3}{c|}{\textbf{ABC} \texttt{if -g}} 
% & \multicolumn{3}{c|}{\textbf{Ours}}  \\
% &Area&Delay&Time&Area&Delay&Time\\
% \hline
%   adder & 1353.26 & 1289.66 & 1.17 & 2066.86 & 659.11 & 16.20  \\ \hline
%         max & 2892.91 & 1922.03 & 1.24 & 2729.61 & 1663.94 & 7.33  \\ \hline
%         square & 15266.78 & 1770.21 & 4.06 & 21687.34 & 1930.33 & 13.38  \\ \hline
%         %arbiter & 5629.05 & 428.24 & 2.4 & 8457.33 & 727.95 & 6.85  \\ \hline
%         sqrt & 35321.16 & 75204.72 & 29.28 & 23122.01 & 87456.66 & 14.93  \\ \hline
%         log2 & 33979.1 & 5675.13 & 10.6 & 25969.9 & 5228.17 & 12.12  \\ \hline
%         div & 64276.34 & 41954.75 & 24.54 & 63367.01 & 48799.02 & 26.01  \\ \hline
%         hyp & 285441.19 & 417583.56 & 145.44 & 200680.28 & 347414.25 & 96.15  \\ \hline
%         multiplier & 27141.43 & 2799.76 & 5.79 & 25069.9 & 3350.99 & 8.94  \\ \hline
%         mem\_ctrl & 33544.96 & 1590.51 & 6.88 & 32422.19 & 1744.66 & 14.06  \\ \hline
%         AVG & 50484.618 & 55021.857 & 23.093 & 40487.096 & 50030.355 & 19.952  \\ \hline
%         Impr & ~& ~ & ~ & \textbf{26.9\%} & \textbf{6.5\%} & \textbf{13.6\%}  \\ \hline
% \hline
% \end{tabular}}
% \label{tab:comparison}
% \end{table}


        % adder & 1353.26 & 1289.66 \\ \hline
        % max & 2892.91 & 1922.03 \\ \hline
        % square & 15266.78 & 1770.21 \\ \hline
        % arbiter & 5629.05 & 428.24 \\ \hline
        % sqrt & 35321.16 & 75204.72 \\ \hline
        % log2 & 33979.1 & 5675.13 \\ \hline
        % div & 64276.34 & 41954.75 \\ \hline
        % hyp & 285441.19 & 417583.56 \\ \hline
        % multiplier & 27141.43 & 2799.76 \\ \hline
        % mem\_ctrl & 33544.96 & 1590.51 \\ \hline
        % AVG & 50484.618 & 55021.857 \\ \hline

==> tables/qor_table.tex <==
\begin{table*}
    \caption{QoR and runtime comparison between \deftextEsynTurbo and the baseline.}
    %\guangyu{It seems `improvements' using geomean to count? Maybe we should illustrate this when we mention xx\%} \guangyu{This table is still updating... (the balanced part will be removed later)}
    %RESULTS COMPARING OUR APPROACH AGAINST STANDARD ABC. $\triangle$ MEANS THE CORRESPONDING VALUES OF $\triangle$ \deftextEsyn $/ A B C$. WE HIGHLIGHT OUR METHOD CAN BEAT THE STANDARD ABC SYNTHESIS FLOW IN DELAY AND AREA FOR ALL THE TEST-CASES. COMPARED TO ABC, WE IMPROVE UP TO 13 OUT OF 13 CASES.}
    \centering
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{l|rrrr|rrrr|rrrc}
    \hline
    \multicolumn{1}{c|}{\multirow{2}{*}{Circuit}} &
    \multicolumn{4}{c|}{\textbf{\textit{SOP Balancing Baseline}} } & 
    \multicolumn{4}{c|}{\textbf{\textit{SOP Balancing  + \deftextEsynTurbo w/o ML model}}} & 
    \multicolumn{4}{c}{\textbf{\textit{SOP Balancing  + \deftextEsynTurbo w ML model}}}
    
    \\ \cline{2-13} 
     &
    \multicolumn{1}{c}{Area ($\mu m^2$)} & 
    \multicolumn{1}{c}{Delay ($ps$)} & 
    \multicolumn{1}{c}{lev } & 
    \multicolumn{1}{c|}{runtime ($s$)} & 
    \multicolumn{1}{c}{Area ($\mu m^2$)} & 
    \multicolumn{1}{c}{Delay ($ps$)} & 
    \multicolumn{1}{c}{lev } & 
    \multicolumn{1}{c|}{runtime ($s$)} & 
    \multicolumn{1}{c}{Area ($\mu m^2$)} & 
    \multicolumn{1}{c}{Delay ($ps$)} & 
    \multicolumn{1}{c}{lev } & 
    \multicolumn{1}{c}{runtime ($s$)}
 \\
    \hline
      hyp & 370305.16 & 253779.06 & 10929 & 1496.23 & 386483.84 & 240435.12 & 10948 & 2102.52 & 366751.38 & 248781.94 & 11033 & 1646.86  \\ \hline
    div & 56873.2 & 25378.59 & 1258 & 108.04 & 34475.98 & 24747.77 & 1300 & 280.79 & 48386.24 & 24333.65 & 1298 & 147.77  \\ \hline   
    mem\_ctrl & 29433.64 & 1281.99 & 61 & 76.5 & 29219.49 & 1056.09 & 59 & 113.17 & 29365.29 & 1081.48 & 60 & 97.09  \\ \hline        
    log2 & 41154.32 & 5233.86 & 231 & 161.49 & 32840.69 & 5033.46 & 240 & 289.79 & 41234.11 & 5153.74 & 233 & 208.30   \\ \hline
multiplier & 35799.38 & 2632.08 & 147 & 54.68 & 31443.34 & 2371.24 & 130 & 105.02 & 35002.03 & 2599.37 & 147 & 87.15  \\ \hline
        sqrt & 53262.02 & 78627.99 & 3574 & 112.27 & 33852.66 & 72796.83 & 3578 & 270.21 & 48909.25 & 76432.02 & 3579 & 143.43  \\ \hline

    square & 21240.14 & 834.01 & 69 & 25.12 & 21418.84 & 792.09 & 69 & 50.22 & 21532.44 & 794.16 & 70 & 37.46  \\ \hline
    arbiter & 4464.75 & 288.18 & 23 & 12.58 & 4587.45 & 270.98 & 22 & 23.34 & 4532.63 & 284.27 & 24 & 20.18  \\ \hline
    sin & 16052.7 & 3712.41 & 119 & 34.95 & 15737.77 & 3567.12 & 113 & 62.31 & 15737.77 & 3685.34 & 118 & 50.83  \\ \hline

    adder & 1206.99 & 584.53 & 57 & 1.96 & 1282.11 & 536.42 & 57 & 10.2 & 1285.61 & 546.86 & 57 & 7.07  \\ \hline
        GEOMEAN & 25274.02 & 5620.01 & 292.93 & 60.32 & 22104.32 & 5210.55 & 287.17 & 126.25 & 24660.84 & 5390.13 & 295.16 & 91.42  \\ \hline
Improvements &             &             &             &  &\textbf{12.54\%}             &    \textbf{7.29\%}           &  &            & \textbf{2.42\%} & \textbf{4.09\%}  & &  \\ \hline
\end{tabular}}
\label{tab:all-results}

%\guangyu{mention https://cn.overleaf.com/project/650becdfc2f93692784f5dc6\deftextEsyn difference with reg or without reg: compare with the original cost function}
\end{table*}

==> tables/runner_delay_operator_setting.tex <==
% \begin{table}[H]
% \centering
% \caption{The Random Parameter For Design Space Exploration.}
% \label{tab:dse_iter} 
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{c||c|c|c}
% \hline 
% Phase& Hyper-Parameter&\textit{w.} Random& \textit{w.o.} Random \\
% \hline \hline 
% Rewrite& \#.Iteration&$[3,30,60,90]$& Determined by \textit{Early-Stop}\\
% \hline
% \multirow{3}{*}{Extract} & Extractor Type&$[$Tree-based, DAG-based$]$& Tree-based \\
% \cline{2-4}
% & Random Probability& $[0,0.1,0.2,0.3]$& 0 \\
% \cline{2-4}
% & Cost Function& [Size, Depth]& Depth\\
% \cline{2-4}
% & \#.Extract Circuit & 20 & 1 \\
% \hline
% \multirow{2}{*}{Fuzzing} & \#. Fuzzing Passes & 400 & 500 \\
% \cline{2-4}
% & Length of Passes & 15-20 & 15-20 \\
% \hline
% \end{tabular}}
% \end{table}

% \begin{table}[H]
% \centering
% \caption{The parameter for design space exploration. We randomly selected 400 circuits generated by different hyper-parameter in \deftextEsynTurbo, comparing ABC's hyper-volumn by optimization passes fuzzing.}
% \label{tab:dse_iter} 
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{c||c|c|c}
% \hline 
% Phase& Hyper-Parameter&\deftextEsynTurbo \textit{w.} Tuning& ABC\\
% \hline \hline 
% Rewrite& \#.~Iteration&$[3,30,60,90]$& -\\
% \hline
% \multirow{3}{*}{Extract} & Extractor Type&$[$\textit{Tree}-based, \textit{DAG}-based$]$& -\\
% \cline{2-4}
% & Random Probability& $[0,0.1,0.2,0.3]$& -\\
% \cline{2-4}
% & Cost Function& $[Size, Depth]$& -\\
% \cline{2-4}
% & \#. Extract Circuit& 20 & - \\
% \hline
% \multirow{2}{*}{Opt. Fuzzing} 
% & \#. Fuzzing Passes per Circuit & 20 & 500 \\
% \cline{2-4}
% & \#. Fuzzing Passes in Total & $\textcolor{teal}{400}~(20~Cric *20~Passes)$ & $500~(1~Circ *500~Passes)$\\
% \cline{2-4}
% & Length of Passes & \textcolor{teal}{10-15} & 15-20 \\
% \hline
% \end{tabular}}

% % \begin{tablenotes}
% % \item $^\star$ There is only one circuit to test different passes.
% % \end{tablenotes}
% \label{table:dse-tuning}
% \end{table}

\begin{table}[!tb]
\centering
\caption{The parameter of \deftextEsynTurbo in runtime-oriented mode (w. Early-Stop) vs. static runtime limit (w/o Early-Stop) for delay optimization.}
%for delay-oriented optimization in a runtime mode w \textit{Early-Stop} and w/o \textit{Early-Stop}.}
\label{tab:early_stop_effect} 
\resizebox{\columnwidth}{!}{
\begin{tabular}{c||c|c|c}
\hline 
Phase& Hyper-Parameter&\deftextEsynTurbo w. \textit{Early-Stop}&\deftextEsynTurbo w/o \textit{Early-Stop} \\
\hline \hline 
\multirow{3}{*}{Rewrite} & Sample Intervals &1 or 2 or 5&-\\
\cline{2-4}
& \#. of Sample Intervals per Checkpoint & $4$&-\\
\cline{2-4}
&Runtime limit& -&$300s$\\
\cline{2-4}
&\#.~Iteration& Determined by \textit{Early-Stop Strategy}&Determined by \textit{runtime limits}\\

\hline
\multirow{3}{*}{Extract} & Extractor Type&$\textit{Tree}$-based&$\textit{Tree}$-based\\
\cline{2-4}
& Random Probability& $w./o~Random$& $w./o~Random$\\
\cline{2-4}
& Cost Function& $Depth$& $Depth$\\
\hline
% & \#. Fuzzing Passes per Circuit & 20 & 500 \\
% \cline{2-4}
%\hline
\end{tabular}}

% \begin{tablenotes}
% \item $^\star$ There is only one circuit to test different passes.
% \end{tablenotes}
\label{table:delay_runner}
\end{table}

==> tables/scale_comp_table.tex <==
% \begin{table}[H]
% \centering
% \caption{Scalability comparison with previous work.}
% \label{table:comp-scale}
% \resizebox{0.8\linewidth}{!}{
% \begin{tabular}{@{}llll}
% \toprule
% Tools  &Max Circuit&\#. aig size & \#. level \\ \midrule
% E-Syn~\cite{chen2024syn}            & arbiter~\cite{}& 11839     & 87      \\
% \deftextEsynTurbo            &hyp~\cite{}&214335     &24801     \\
%            \bottomrule

% \end{tabular}}
% \begin{tablenotes}
% \item $^\star$ Both designs are from EPFL benchmark~\cite{}
% \end{tablenotes}  
% \end{table}

% \begin{table}[]
%     \centering
% \resizebox{0.8\linewidth}{!}{
% \begin{tabular}{l|l||c|c|c}
% \hline \multirow{2}{*}{ Tool } & \multirow{2}{*}{ Benchmarks} & \multirow{2}{*}{ \#Designs } & \multicolumn{2}{c}{ Design Size Range } \\
% \cline { 4 - 5 } & & & \#. AIG Size & \#. Levels \\
% \hline \hline \multirow{7}{*}{Esyn~\cite{chen2024syn}} & EPFL & 4 & $9-45$ & $0.4-1.3$ \\
% \cline { 2 - 5 } & ISCAS'85~\cite{}$^{\star}$ & 2 & - & - \\
% \cline { 2 - 5 } & LGSynth'91~\cite{}$^{\star}$ & 2 & - & - \\
% \cline { 2 - 5 } & LGSynth'89~\cite{} & 2 & - & - \\
% \cline { 2 - 5 } & ITC'99~\cite{} & 1 & - & - \\
% \cline { 2 - 5 } & OpenCores~\cite{} & 1 & - & - \\
% \cline { 2 - 5 } & GenMul~\cite{} & 2 & - & - \\
% \hline EsynTurbo & EPFL~\cite{} & 20 & - & - \\
% \hline
% \end{tabular}}
% \begin{tablenotes}
% \item $^\star$ Both designs are from EPFL benchmark~\cite{}
% \end{tablenotes}
% \end{table}


\begin{table}
\centering
\caption{Scalability comparison with the previous work. Although \deftextEsyn~\cite{chen2024syn} was tested using circuits from a range of benchmarks, the design scales were much smaller, compared to this work.}
\label{table:comp-scale}
\resizebox{\linewidth}{!}{
\begin{tabular}{l|l||c|c|c|c}
\hline \multirow{2}{*}{ Tool } & \multirow{2}{*}{ Benchmarks} & \multirow{2}{*}{ \#. Designs } & \multicolumn{2}{|c|}{ Design Size Range } & \multirow{1}{*}{ Scalability} \\
\cline { 4 - 6 } & & & \#. AIG node (k)& \#. level (k)& >10k AIG nodes\\
\hline \hline \multirow{7}{*}{DAC 24~\cite{chen2024syn}} & EPFL~\cite{amaru2015epfl}  & 4/23 & 0.693 - 3.336& 0.016 - 0.287& \multirow{7}{*}{\textcolor{red}{$\times$}} \\
\cline { 2 - 5 } & ISCAS'85~\cite{brglez1985neutral} & 2/11 & 0.718 - 2.192& 0.022 - 0.030& \\
\cline { 2 - 5 } & LGSynth'91~\cite{yang1991logic} & 2/116 & 0.763 - 1.811& 0.007 - 0.037& \\
\cline { 2 - 5 } & LGSynth'89~\cite{yang1989logic} & 2/64 & 0.212 - 1.233& 0.015 - 0.043& \\
\cline { 2 - 5 } & ITC'99~\cite{corno2000rt} & 1/28 & 1.01& 0.022& \\
\cline { 2 - 5 } & OpenCores & 1 & 1.81& 0.027&  \\
\cline { 2 - 5 } & GenMul~\cite{mahzoon2021genmul} & 2 & 0.054 - 0.19& 0.013 - 0.039& \\
\hline \deftextEsynTurbo & EPFL~\cite{amaru2015epfl} & \textcolor{teal}{20/23}$^{\star}$ & \textcolor{teal}{0.174 - 214.335}& \textcolor{teal}{0.003 - 24.801}& %\textcolor{teal}{$\halfcheckmark$} \\
\textcolor{teal}{$\checkmark$} \\
\hline
\end{tabular}}
\begin{tablenotes}
% \item $^\star$ Design from a fixed point math library for Verilog
\item $^\star$ \footnotesize{including \textbf{arithmetic} and \textbf{random/control} benchmarks.} %\textbf{MtM (More than ten Million gates)} benchmarks are not tested.
%\footnote{https://opencores.org/projects/verilog\_fixed\_point\_math\_library}
\end{tablenotes}
\end{table}

        % adder & 1353.26 & 1289.66 \\ \hline
        % max & 2892.91 & 1922.03 \\ \hline
        % square & 15266.78 & 1770.21 \\ \hline
        % arbiter & 5629.05 & 428.24 \\ \hline
        % sqrt & 35321.16 & 75204.72 \\ \hline
        % log2 & 33979.1 & 5675.13 \\ \hline
        % div & 64276.34 & 41954.75 \\ \hline
        % hyp & 285441.19 & 417583.56 \\ \hline
        % multiplier & 27141.43 & 2799.76 \\ \hline
        % mem\_ctrl & 33544.96 & 1590.51 \\ \hline
        % AVG & 50484.618 & 55021.857 \\ \hline

==> tables/total.tex <==
\begin{table*}[!tb]
    \centering
    % \caption{The QoR and runtime comparison among commonly-used operators (\texttt{dc2} and \texttt{dch}) in \texttt{ABC}, and \deftextEsynTurbo. \deftextEsynTurbo is in the runtime-oriented mode.
    % Light green indicates that \deftextEsynTurbo performs better as a hybrid operator comparing with the Lazyman Synthesis Flow baseline.}
    \caption{}
\label{total} 
    \resizebox{\linewidth}{!}{
    \renewcommand{\arraystretch}{1.5}  % Increase vertical spacing default 1.2
    \setlength{\tabcolsep}{8pt}  % Increase horizontal spacing, default 5
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c||c|}
    \hline
         \multicolumn{3}{|c|}{\textbf{Design}} & \textit{adder} & \textit{sin}& \textit{square} & \textit{arbiter} & \textit{sqrt} & \textit{log2} & \textit{div} & \textit{hyp} & \textit{multiplier} & \textit{mem\_ctrl} & \textbf{GEOMEAN}\\
         
         \hline \hline
         
        \multirow{3}{*}{\textbf{\textit{\textcolor{blue}{SOP Balancing Synthesis Flow}}}}& \multicolumn{2}{c|}{\textbf{Area ($\mu m^2$)}} & & 17180.61& 21039.76& 4464.75& 53262.02& 45588.98& 56873.2&370305.16
 & 35799.38& 28808.91& \\ \cline{2-14}
         & \multicolumn{2}{c|}{ \textbf{Delay($ps$)}} & & 3457.54& 801.16& 288.18& 78627.99& 5798.41& 25378.59& 253779.06& 2632.08& 1251& \\ \cline{2-14}
        & \multicolumn{2}{c|}{ \textbf{Lev}} & & 116& 68& 23& 3574& 231& 1258& 10929& 147& 62& \\ \cline{2-14}
         & \multicolumn{2}{c|}{\textbf{runtime($s$)}} & & 31.97& 23.27& 12.58& 109.41& 161.49& 108.04&1496.23 & 54.68& 71.29& \\ \hline
         
         \multirow{3}{*}{\textbf{\textit{\textcolor{blue}{SOP Balancing} + \deftextEsynTurbo} (\textcolor{red}{Ours})}}& \multicolumn{2}{c|}{\textbf{Area ($\mu m^2$)}} & & \textbf{8045.36}&  21448.93& \textbf{4587.45}& 33239.13& \textbf{32840.69}& \textbf{40415.06}& & \textbf{31443.34}& 30178.03& \\ \cline{2-14}
         & \multicolumn{2}{c|}{ \textbf{Delay($ps$)}} & & \textbf{2998.27}&  789.84& \textbf{270.98}&\textbf{77980.27} & \textbf{5033.46}& \textbf{24947.49}&& \textbf{2371.24}& \textbf{1158.1}& \\ \cline{2-14}
        & \multicolumn{2}{c|}{ \textbf{Lev}} & & \textbf{113}& 68& \textbf{22}& \textbf{3500}& 240& 1301& & \textbf{130}& \textbf{56}& \\ \cline{2-14}
         & \multicolumn{2}{c|}{\textbf{runtime($s$)}} & & \textbf{12.13}& & \textbf{8.07}& \textbf{57.47}& \textbf{57.95}& 151.63& & \textbf{37.36}& \textbf{28.27}& \\ \hline
         
         \multirow{3}{*}{\textbf{\textit{\textcolor{blue}{SOP Balancing} + }DAC'24~\cite{chen2024syn}}}& \multicolumn{2}{c|}{\textbf{Area ($\mu m^2$)}} & & & & & & & & & & & \\ \cline{2-14}
         & \multicolumn{2}{c|}{ \textbf{Delay($ps$)}} & & & & & & & & & & & \\ \cline{2-14}
        & \multicolumn{2}{c|}{ \textbf{Lev}} & & & & & & & & & & & \\ \cline{2-14}
         & \multicolumn{2}{c|}{\textbf{runtime($s$)}} & & & & & & & & & & & \\ 

    \hline
    \hline
    
       % \multirow{3}{*}{\textbf{\textit{\textcolor{orange}{Lazyman Synthesis Flow}}}} & \multicolumn{2}{c|}{\textbf{Area ($\mu m^2$)}} & 37392.22 & 25542.06 & 50857.61 & 1260.18 & 27179.42 & 3303.76 & 64844.84 & 62457.69 & & & \\ \cline{2-14}
       %  ~ & \multicolumn{2}{c|}{ \textbf{Delay($ps$)}} & 53939.85 & 1078.66 & 3046.02 & 785.28 & 1449.36 & 2318.81 & 33813.79 & 6965.71 & & & \\ \cline{2-14}
       %  ~ & \multicolumn{2}{c|}{\textbf{runtime($s$)}} & 44.38 & 21.509 & 38.54 & 1.43 & 33.13 & 3.76 & 119.04 & 128.57 & & & \\ \hline
       % \multirow{3}{*}{\textbf{\textit{\textcolor{orange}{Lazyman} + }DAC'24~\cite{chen2024syn}}}& \multicolumn{2}{c|}{\textbf{Area ($\mu m^2$)}} & \cellcolor[rgb]{0.77, 0.87, 0.71}37127.91 & 28062.65 & \cellcolor[rgb]{0.77, 0.87, 0.71}50118.57 & 1271.84 & 27313.59 & \cellcolor[rgb]{0.77, 0.87, 0.71}2932.56 & \cellcolor[rgb]{0.77, 0.87, 0.71}60673.79 & \cellcolor[rgb]{0.77, 0.87, 0.71}53606.81 & 12200.54 & & \\ \cline{2-14}
       %  {} & \multicolumn{2}{c|}{ \textbf{Delay($ps$)}} & \cellcolor[rgb]{0.77, 0.87, 0.71}46747.29 & \cellcolor[rgb]{0.77, 0.87, 0.71}871.15 & \cellcolor[rgb]{0.77, 0.87, 0.71}2677.89 & \cellcolor[rgb]{0.77, 0.87, 0.71}649.96 & \cellcolor[rgb]{0.77, 0.87, 0.71}1153.84 & \cellcolor[rgb]{0.77, 0.87, 0.71}1350.11 & \cellcolor[rgb]{0.77, 0.87, 0.71}32204.6 & \cellcolor[rgb]{0.77, 0.87, 0.71}5062.9 & \cellcolor[rgb]{0.77, 0.87, 0.71}3544.3 & & \\ \cline{2-14}
       %   & \multicolumn{2}{c|}{\textbf{runtime($s$)}} & 637.79 & 39.33 & 81.2 & 7.52 & 46.874 & 11.193 & 998.45 & 193.28 & 21.396 & & \\ \hline
       %   \multirow{3}{*}{\textbf{\textit{\textcolor{orange}{Lazyman} + \deftextEsynTurbo} (\textcolor{red}{Ours}) }}& \multicolumn{2}{c|}{\textbf{Area ($\mu m^2$)}} & & & & & & & & & & & \\ \cline{2-14}
       %   & \multicolumn{2}{c|}{ \textbf{Delay($ps$)}} & & & & & & & & & & & \\ \cline{2-14}
       %   & \multicolumn{2}{c|}{\textbf{runtime($s$)}} & & & & & & & & & & & \\ \hline
    \end{tabular}}
\end{table*}

==> tables/total_deprecated.tex <==
\begin{table*}[!tb]
    \centering
    \caption{The QoR and runtime comparison among commonly-used operators (\texttt{dc2} and \texttt{dch}) in \texttt{ABC}, and \deftextEsynTurbo. \deftextEsynTurbo is in the runtime-oriented mode.
    Light blue indicates that \deftextEsynTurbo, as a standalone optimization operator, achieves the optimal QoR comparing with \texttt{dc2} and \texttt{dch}. Light green indicates that \deftextEsynTurbo performs better as a hybrid operator comparing with either \texttt{dc2} or \texttt{dch} operator alone. 7nm and 130nm denote ASAP 7nm and SkyWater 130nm technology library, respectively.}
    % \cchen{improvement data in figs/source/total.csv}}
    %For each case, the result measurements are presented in two rows: the first row corresponds to the results for the ASAP 7nm technology library, while the second row represents the results for the SkyWater 130nm technology library.}
\label{total} 
    \resizebox{\linewidth}{!}{
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c||c|}
    \hline
         \multicolumn{3}{|c|}{\textbf{Design}} & cavlc & int2 & sqrt & dec & square & mul & voter & prio & arbi & adder & mem & hyp & max & router & div & log2 & i2c & ctrl & bar & sin & \textbf{GEOMEAN}\\ \hline
        \hline
        \multirow{8}{*}{\textbf{\textit{dc2}}} & \multicolumn{2}{c|}{\textbf{and}} & 649 & 208 & 18452 & 304 & 16676& 24377 & 8597 & 703 & 11839 & 1019 & 42755 & 211688 & 2833 & 223 & 40443 & 29323 & 1136 & 96 & 2952 & 5040&3712.18 \\ \cline{2-24}
        &  \multirow{2}{*}{\textbf{Area ($\mu m^2$)}}& \textbf{7nm} & 475.19 & 153.5 & 19753.22 & 351.55 & 15679.45 & 21977.31 & 11681.96 & 791.05 & 7758.19 & 1157.07 & 29303 & 212334.25 & 2420.98 & 218.58 & 47284.22 & 26513.44 & 819.75 & 100.31 & 2302.47 & 5873.52&3476.39\\ \cline{3-24}
         & &\textbf{130nm} & 2319.72 & 800.77 & 90505.55 & 1705.39 & 66532.56 & 94844.71 & 51719.6 & 3218.09 & 43286.52 & 4858.41 & 132345.67 & 920570.38 & 11019.32 & 1103.56 & 188454.48 & 112223.88 & 3827.42 & 419.15 & 10747.81 & 24450.95&15708.13 \\ \cline{2-24}
        & \multicolumn{2}{c|}{\textbf{lev}} & 17 & 13 & 6065 & 3 & 248 & 262 & 59 & 216 & 89 & 255 & 98 & 24873 & 213 & 26 & 4397 & 358 & 14 & 7 & 14 & 161&119.53 \\ \cline{2-24}
         & \multirow{2}{*}{ \textbf{Delay($ps$)}}& \textbf{7nm} & 128.3 & 101.89 & 81114.03 & 69.63 & 3042.11 & 3315.69 & 818.28 & 2121.13 & 849.17 & 2723.03 & 1604.31 & 470401.34 & 2798.07 & 282.13 & 69860.64 & 4540.24 & 242.62 & 49.83 & 291.88 & 2643.51& 1534.92\\ \cline{3-24}
         && \textbf{130nm}  & 837.63 & 581.22 & 390184.28 & 402.39 & 15273.2 & 17530.65 & 4415.2 & 13069.15 & 4629.53 & 15022.15 & 8569.68 & 1831879.12 & 13826.68 & 1426.21 & 316733.59 & 25561.53 & 1041.29 & 337.98 & 1498.7 & 12836.06& 8076.21\\ \cline{2-24}
         & \multirow{2}{*}{\textbf{runtime($s$)}}& \textbf{7nm} & 0.62 & 0.66 & 4.57 & 0.86 & 2.13 & 4.72 & 1.83 & 0.61 & 4.25 & 0.82 & 5.52 & 71.8 & 0.91 & 0.64 & 9.04 & 9.23 & 0.85 & 0.56 & 1.22 & 1.67& 2.01\\ \cline{3-24}
         & & \textbf{130nm} & 0.33 & 0.26 & 14.11 & 0.27 & 2.29 & 5.06 & 1.99 & 0.43 & 4.38 & 0.3 & 6.08 & 116.61 & 1 & 0.21 & 11.17 & 7.56 & 0.4 & 0.24 & 0.68 & 1.59&1.54 \\ \hline
         \multirow{8}{*}{\textbf{\textit{dch}}} & \multicolumn{2}{c|}{\textbf{and}} & 639 & 207 & 19326 & 304 & 16640 & 24579 & 8583 & 670 & 11840 & 1019 & 41728 & 211694 & 2831 & 201 & 30808 & 29039 & 1095 & 91 & 2952 & 5023&3616.55 \\ \cline{2-24}
        & \multirow{2}{*}{\textbf{Area ($\mu m^2$)}}& \textbf{7nm} & 489.65 & 170.99 & 24172.71 & 351.55 & 15925.79 & 22475.13 & 12473.01 & 639.65 & 7893.03 & 1258.55 & 28652.85 & 203284.62 & 2510.79 & 202.49 & 34323.19 & 28396.24 & 808.32 & 96.11 & 2416.31 & 6027.96 &3474.97 \\ \cline{3-24}
        &  & \textbf{130nm}& 2282.19 & 731.95 & 110313.3 & 1705.39 & 67123.12 & 97922.66 & 52694.29 & 3687.29 & 44581.51 & 6902.87 & 129651.84 & 892318.31 & 10023.36 & 980.94 & 137819.67 & 121204.99 & 3723.57 & 427.91 & 10651.47 & 25126.6&15849.55 \\ \cline{2-24}
        & \multicolumn{2}{c|}{\textbf{lev}} & 13 & 10 & 4969 & 3 & 248 & 262 & 55 & 202 & 87 & 255 & 91 & 24689 & 163 & 23 & 4375 & 362 & 14 & 7 & 12 & 158&110.74 \\ \cline{2-24}
         & \multirow{2}{*}{ \textbf{Delay($ps$)}}& \textbf{7nm} & 120.55 & 79.18 & 106864.79 & 69.63 & 3014.28 & 3293.72 & 850.29 & 1930.24 & 951.68 & 2901.95 & 1642.43 & 357287.09 & 1907.32 & 228.37 & 67410.44 & 4794.31 & 172.99 & 48.29 & 243.64 & 2705.22&1439.21 \\ \cline{3-24}
        & & \textbf{130nm}& 728.95 & 518.61 & 460257.12 & 402.39 & 15182.22 & 17361.96 & 4332.19 & 12428.5 & 4339.93 & 15328.44 & 7635.35 & 2409397.75 & 11391.95 & 1313.1 & 319761.81 & 24411.71 & 918.09 & 332.2 & 1414.86 & 13010.84&7853.79 \\ \cline{2-24}
         & \multirow{2}{*}{\textbf{runtime($s$)}}& \textbf{7nm} & 0.9 & 0.72 & 9.93 & 0.81 & 3.28 & 5.4 & 3.41 & 0.67 & 9.28 & 0.83 & 12.59 & 1026.52 & 0.89 & 0.6 & 16.92 & 12.59 & 0.77 & 0.98 & 1.17 & 3.08 &3.09\\ \cline{3-24}
         & & \textbf{130nm} & 0.35 & 0.26 & 12.02 & 0.27 & 3.09 & 5.51 & 3.69 & 0.57 & 6.99 & 0.69 & 11.93 & 786.7 & 0.78 & 0.27 & 12.42 & 12 & 0.43 & 0.23 & 0.73 & 2.37&2.09 \\ \hline
    
       \multirow{10}{*}{\textbf{\deftextEsynTurbo}} & \multirow{2}{*}{\textbf{and}}& \textbf{7nm} & 749 & 280 & 25110 & 310 & 25899 & 31269.32 & 13760 & 1012 & 11967 & 1889 & 46862 & 215223 & 3010 & 504 & 57359 & 32060 & 1538 & 156 & 3430 & 5871&4871.15  \\ \cline{3-24}
         & & \textbf{130nm} & 749 & 280 & 25110 & 308 & 25899 & 27062 & 13758 & 2309 & 12092 & 1429 & 47859 & 215223 & 3492 & 505 & 57305 & 32060 & 1538 & 158 & 3464 & 5416 &4998.87 \\ \cline{2-24}
        ~ & \multirow{2}{*}{\textbf{Area ($\mu m^2$)}}& \textbf{7nm} & 544.48 & 202.02 & 23132.28 & 354.82 & 21687.34 & 37124 & 19507.81 & 808.08 & 8457.33 & 1658.62 & 32422.19 & 214098.55 & 2352.4 & 443.7 & 63028.05 & 25969.9 & 1072.62 & 127.37 & 2989.25 & 5475.55&4280.39 \\ \cline{3-24}
        & & \textbf{130nm}&2492.39 & 930.89 & 132365.7 & 1761.69 & 96283.59 & 105491.17 & 5380.69 & 7644.83 & 38515.69 & 6528.76 & 148237.17 & 1026042.81 & 12256.75 & 1906.83 & 260888.95 & 111319.27 & 4939.74 & 750.72 & 11039.34 & 22562.89&17246.5  \\ \cline{2-24}
        ~ & \multirow{2}{*}{\textbf{lev}}& \textbf{7nm} & \cellcolor{lightblue}{12} & \cellcolor{lightblue}10 & \cellcolor{lightblue}5057 & 4 & \cellcolor{lightblue}225 & \cellcolor{lightblue}260 & 70 & 250 & \cellcolor{lightblue}87 & \cellcolor{lightblue}129 & 114 & \cellcolor{lightblue}24801 & 253 & 30 & \cellcolor{lightblue}4372 & 444 &\cellcolor{lightblue} 13 &\cellcolor{lightblue} 6 & \cellcolor{lightblue}12 & 215&117.07  \\ \cline{3-24}
        ~ & & \textbf{130nm}&\cellcolor{lightblue}12 &\cellcolor{lightblue} 10 & \cellcolor{lightblue}5057 & \cellcolor{lightblue}3 & \cellcolor{lightblue}225 & 274 & 70 & \cellcolor{lightblue}187 & \cellcolor{lightblue}87 & \cellcolor{lightblue}193 & 114 & \cellcolor{lightblue}24801 & 224 & 30 & \cellcolor{lightblue}4372 & 444 & \cellcolor{lightblue}13 &\cellcolor{lightblue} 6 &\cellcolor{lightblue} 12 & 225 &115.91 \\ \cline{2-24}
        ~ & \multirow{2}{*}{ \textbf{Delay($ps$)}}& \textbf{7nm} & \cellcolor{lightblue}104.99 & \cellcolor{lightblue}74.38 & 87412.19 & \cellcolor{lightblue}68.65 & \cellcolor{lightblue}1930.33 &\cellcolor{lightblue} 3084.94 & 1049.23 & 2094.23 & \cellcolor{lightblue}727.95 & \cellcolor{lightblue}1135.55 & 1744.66 & \cellcolor{lightblue}352762.5 & 2488.61 & 252.85 & \cellcolor{lightblue}51098.14 & 5228.17 & \cellcolor{lightblue}118.5 & 57.15 & 276.28 & 2802.91&\cellcolor{lightblue}1324.24 \\ \cline{3-24}
        ~ & & \textbf{130nm} &\cellcolor{lightblue}717.98 & 526.79 & 486174.06 & \cellcolor{lightblue}370.33 & \cellcolor{lightblue}12786.64 & 18334.21 & 5380.69 & \cellcolor{lightblue}11851.7 & 4607.9 &\cellcolor{lightblue} 8648.72 & 9261.86 & \cellcolor{lightblue}1788036.25 & 13259.45 & 1562.27 & 328461.03 & 28182.71 & \cellcolor{lightblue}733.52 & \cellcolor{lightblue}297.11 & 1501.11 & 13723.56& \cellcolor{lightblue}7728.81\\ \cline{2-24}
        ~ & \multirow{2}{*}{\textbf{runtime($s$)}}& \textbf{7nm} & 3.47 & 2.41 & 16.14 & 1.99 & 14.29 & 24.64 & 3.29 & 3.33 & 8.7 & 5.96 & 14.32 & 133.86 & 3.27 & 2.37 & 27.55 & 13.59 & 3.9 & 1.86 & 3.57 & 4.33 &6.7\\ \cline{3-24}
        ~ & & \textbf{130nm} & 3.72 & 2.06 & 25.67 & 1.53 & 14.75 & 14.88 & 6.63 & 3.98 & 11.61 & 1.99 & 14.63 & 154.5 & 4.29 & 2.27 & 27.86 & 14.54 & 3.32 & 1.93 & 2.59 & 4.43&6.62 \\ \hline
        \hline


        
       &\multirow{2}{*}{ \textbf{and}}& \textbf{7nm}& \cellcolor[rgb]{0.77, 0.87, 0.71}645 & \cellcolor[rgb]{0.77, 0.87, 0.71}202 & 18464 & \cellcolor[rgb]{0.77, 0.87, 0.71}304 & 16902 & \cellcolor[rgb]{0.77, 0.87, 0.71}24375 & 8630 & 734 & \cellcolor[rgb]{0.77, 0.87, 0.71}11839 & 1254 & 42831 & 212742 &\cellcolor[rgb]{0.77, 0.87, 0.71} 2833 &\cellcolor[rgb]{0.77, 0.87, 0.71} 185 & \cellcolor[rgb]{0.77, 0.87, 0.71}40431 & \cellcolor[rgb]{0.77, 0.87, 0.71}29320 & \cellcolor[rgb]{0.77, 0.87, 0.71}1131 & 110 &\cellcolor[rgb]{0.77, 0.87, 0.71} 2952 & 5051&3746.96 \\ \cline{3-24}
        &  & \textbf{130nm}& \cellcolor[rgb]{0.77, 0.87, 0.71}639 & \cellcolor[rgb]{0.77, 0.87, 0.71}202 & 18465 & \cellcolor[rgb]{0.77, 0.87, 0.71}304 & 17156 & 24379 & 8625 & 1316 &\cellcolor[rgb]{0.77, 0.87, 0.71} 11839 & 1254 & 42831 & 212744 & 2860 &\cellcolor[rgb]{0.77, 0.87, 0.71} 186 & \cellcolor[rgb]{0.77, 0.87, 0.71}40433 & \cellcolor[rgb]{0.77, 0.87, 0.71}29318 &\cellcolor[rgb]{0.77, 0.87, 0.71}1128 & 103 & 2957 & 5071&3849.72 \\ \cline{2-24}
        
       & \multirow{2}{*}{\textbf{Area ($\mu m^2$)}}& \textbf{7nm} & 481.49 & 172.16 & 19856.33 & \cellcolor[rgb]{0.77, 0.87, 0.71}351.55 & 16082.32 & 22240.91 & \cellcolor[rgb]{0.77, 0.87, 0.71}11562.29   & 1006.6 &\cellcolor[rgb]{0.77, 0.87, 0.71} 7679.58 & 1255.75 & 29397.25 & 222647.8 & 2542.99 & \cellcolor[rgb]{0.77, 0.87, 0.71}146.73 & \cellcolor[rgb]{0.77, 0.87, 0.71}46605.61 & 26856.83 & 846.34 & \cellcolor[rgb]{0.77, 0.87, 0.71}95.18 & 2305.51 & \cellcolor[rgb]{0.77, 0.87, 0.71}5735.19&3498.94 \\ \cline{3-24}
       
        {\textbf{\deftextEsynTurbo}} & & \textbf{130nm} & \cellcolor[rgb]{0.77, 0.87, 0.71}2309.72 & \cellcolor[rgb]{0.77, 0.87, 0.71}788.26 &\cellcolor[rgb]{0.77, 0.87, 0.71} 85450.7 & \cellcolor[rgb]{0.77, 0.87, 0.71}1705.39 & 69337.75 & 95835.66 & \cellcolor[rgb]{0.77, 0.87, 0.71}49824.04 & 5438.97 &\cellcolor[rgb]{0.77, 0.87, 0.71} 42131.66 & 5938.2 & \cellcolor[rgb]{0.77, 0.87, 0.71}132330.66 & 973378.5 & \cellcolor[rgb]{0.77, 0.87, 0.71}10645.21 & \cellcolor[rgb]{0.77, 0.87, 0.71}782 & 192225.61 & 115001.55 & 4096.43 & 501.73 & 10780.34 & 24274.53&16186.32 \\ \cline{2-24}
        
        {\textbf{+}} & \multirow{2}{*}{\textbf{lev}}& \textbf{7nm} & \cellcolor[rgb]{0.77, 0.87, 0.71}15 & \cellcolor[rgb]{0.77, 0.87, 0.71}11 & 6068 & \cellcolor[rgb]{0.77, 0.87, 0.71}3 & \cellcolor[rgb]{0.77, 0.87, 0.71}247 & \cellcolor[rgb]{0.77, 0.87, 0.71}262 & 62 & \cellcolor[rgb]{0.77, 0.87, 0.71}215 & \cellcolor[rgb]{0.77, 0.87, 0.71}88 &\cellcolor[rgb]{0.77, 0.87, 0.71} 214 & \cellcolor[rgb]{0.77, 0.87, 0.71}96 & 24874 &\cellcolor[rgb]{0.77, 0.87, 0.71} 206 & \cellcolor[rgb]{0.77, 0.87, 0.71}23 & 4409 & 359 &\cellcolor[rgb]{0.77, 0.87, 0.71} 14 & \cellcolor[rgb]{0.77, 0.87, 0.71}6 &\cellcolor[rgb]{0.77, 0.87, 0.71} 14 & 162&\cellcolor[rgb]{0.77, 0.87, 0.71}115.1 \\ \cline{3-24}
        {\textbf{\textit{{dc2}}}} & & \textbf{130nm} & \cellcolor[rgb]{0.77, 0.87, 0.71}15 & \cellcolor[rgb]{0.77, 0.87, 0.71}11 & \cellcolor[rgb]{0.77, 0.87, 0.71}6057 & \cellcolor[rgb]{0.77, 0.87, 0.71}3 & \cellcolor[rgb]{0.77, 0.87, 0.71}247 &\cellcolor[rgb]{0.77, 0.87, 0.71} 262 & 63 & \cellcolor[rgb]{0.77, 0.87, 0.71}190 & \cellcolor[rgb]{0.77, 0.87, 0.71}89 & \cellcolor[rgb]{0.77, 0.87, 0.71}214 &\cellcolor[rgb]{0.77, 0.87, 0.71} 96 & 24878 & \cellcolor[rgb]{0.77, 0.87, 0.71}182 & \cellcolor[rgb]{0.77, 0.87, 0.71}22 & 4404 &\cellcolor[rgb]{0.77, 0.87, 0.71} 358 & \cellcolor[rgb]{0.77, 0.87, 0.71}14 & \cellcolor[rgb]{0.77, 0.87, 0.71}7 & \cellcolor[rgb]{0.77, 0.87, 0.71}14 & 162&\cellcolor[rgb]{0.77, 0.87, 0.71}114.43 \\ \cline{2-24}
         
         
         & \multirow{2}{*}{ \textbf{Delay($ps$)}}& \textbf{7nm} & \cellcolor[rgb]{0.77, 0.87, 0.71}116.23 & \cellcolor[rgb]{0.77, 0.87, 0.71}77.12 & \cellcolor[rgb]{0.77, 0.87, 0.71}79232.68 &\cellcolor[rgb]{0.77, 0.87, 0.71} 69.63 & \cellcolor[rgb]{0.77, 0.87, 0.71}2174.21 &\cellcolor[rgb]{0.77, 0.87, 0.71} 3280.22 & 825.32 & \cellcolor[rgb]{0.77, 0.87, 0.71}1969.8 & 945.84 &\cellcolor[rgb]{0.77, 0.87, 0.71} 1921.73 &\cellcolor[rgb]{0.77, 0.87, 0.71} 1546.27 & 489135.41 &\cellcolor[rgb]{0.77, 0.87, 0.71} 2179.61 &\cellcolor[rgb]{0.77, 0.87, 0.71} 205.33 & \cellcolor[rgb]{0.77, 0.87, 0.71}66474.01 &\cellcolor[rgb]{0.77, 0.87, 0.71} 4511.33 &\cellcolor[rgb]{0.77, 0.87, 0.71} 145.73 &\cellcolor[rgb]{0.77, 0.87, 0.71} 46.03 & \cellcolor[rgb]{0.77, 0.87, 0.71}284.21 & 2691.62&\cellcolor[rgb]{0.77, 0.87, 0.71}1370.04 \\ \cline{3-24}
         
         & & \textbf{130nm}&\cellcolor[rgb]{0.77, 0.87, 0.71} 732.2 & \cellcolor[rgb]{0.77, 0.87, 0.71}489.19 & 458801.66 & \cellcolor[rgb]{0.77, 0.87, 0.71}402.39 &\cellcolor[rgb]{0.77, 0.87, 0.71} 13728.49 &\cellcolor[rgb]{0.77, 0.87, 0.71} 17122.9 & \cellcolor[rgb]{0.77, 0.87, 0.71}4410.81 &\cellcolor[rgb]{0.77, 0.87, 0.71} 9782.79 & 4765.27 & \cellcolor[rgb]{0.77, 0.87, 0.71}10006.76 & \cellcolor[rgb]{0.77, 0.87, 0.71}8279.15 &\cellcolor[rgb]{0.77, 0.87, 0.71} 1791684.5 & 11817.88 & \cellcolor[rgb]{0.77, 0.87, 0.71}1092.91 &\cellcolor[rgb]{0.77, 0.87, 0.71} 315253.06 & \cellcolor[rgb]{0.77, 0.87, 0.71}24979.49 &\cellcolor[rgb]{0.77, 0.87, 0.71} 772.06 & \cellcolor[rgb]{0.77, 0.87, 0.71}312.9 &\cellcolor[rgb]{0.77, 0.87, 0.71} 1488.6 & \cellcolor[rgb]{0.77, 0.87, 0.71}12747.33&\cellcolor[rgb]{0.77, 0.87, 0.71}7366.15 \\ \cline{2-24}
         
         
         
         & \multirow{2}{*}{\textbf{runtime($s$)}}& \textbf{7nm} & 7.58 & 3.9 & 17.79 & 5.3 & 11.18 & 17.72 & 16.72 & 8.11 & 8.7 & 7.18 & 26.1 & 208.571 & 5.93 & 4.29 & 29.92 & 38.77 & 4.93 & 1.86 & 6.52 & 7.59 &10.63\\ \cline{3-24}
         & & \textbf{130nm} & 3.62 & 1.48 & 19.79 & 1.12 & 12.04 & 16.83 & 5.66 & 3.45 & 9.03 & 3.21 & 14.81 & 188.22 & 4.022 & 2.2 & 30.95 & 19.01 & 1.93 & 1.44 & 4.1 & 4.7&6.33 \\ \hline


         
        &\multirow{2}{*}{\textbf{and}}& \textbf{7nm} & \cellcolor[rgb]{0.77, 0.87, 0.71}638 & \cellcolor[rgb]{0.77, 0.87, 0.71}207 & 19328 &\cellcolor[rgb]{0.77, 0.87, 0.71} 304 & 17022 & 24588 & \cellcolor[rgb]{0.77, 0.87, 0.71}8574 & 851 & \cellcolor[rgb]{0.77, 0.87, 0.71}11311 & 1335 & 42005 & 212696 & 2833 & 209 & 30978 &\cellcolor[rgb]{0.77, 0.87, 0.71} 28787 & 1111 & 115 & \cellcolor[rgb]{0.77, 0.87, 0.71}2952 & 5061&3761.9 \\ \cline{3-24}
        
         & & \textbf{130nm} & \cellcolor[rgb]{0.77, 0.87, 0.71}634 & 208 & 19328 & \cellcolor[rgb]{0.77, 0.87, 0.71}304 & 17159 & 24582 &\cellcolor[rgb]{0.77, 0.87, 0.71} 8574 & 851 & 11857 & 1266 & 41933 & \cellcolor[rgb]{0.77, 0.87, 0.71}212674 & 2837 &\cellcolor[rgb]{0.77, 0.87, 0.71} 175 & \cellcolor[rgb]{0.77, 0.87, 0.71}30796 &\cellcolor[rgb]{0.77, 0.87, 0.71} 28767 & \cellcolor[rgb]{0.77, 0.87, 0.71}1089 & 110 &\cellcolor[rgb]{0.77, 0.87, 0.71} 2952 & 5047&3714.91 \\ \cline{2-24}


         
         & \multirow{2}{*}{\textbf{Area ($\mu m^2$)}}& \textbf{7nm} & 493.62 & \cellcolor[rgb]{0.77, 0.87, 0.71}162.83 & \cellcolor[rgb]{0.77, 0.87, 0.71}24041.6 & \cellcolor[rgb]{0.77, 0.87, 0.71}351.55 & 15730.54 & \cellcolor[rgb]{0.77, 0.87, 0.71}22339.59 &\cellcolor[rgb]{0.77, 0.87, 0.71} 11879.32 & 919.12 & \cellcolor[rgb]{0.77, 0.87, 0.71}7312.16 & 1391.52 & 29004.87 & 208010.64 & \cellcolor[rgb]{0.77, 0.87, 0.71}2386.92 &\cellcolor[rgb]{0.77, 0.87, 0.71} 199.92 & \cellcolor[rgb]{0.77, 0.87, 0.71}34307.09 & 29376.25 & 873.4 & 109.87 & \cellcolor[rgb]{0.77, 0.87, 0.71}2410.72 & \cellcolor[rgb]{0.77, 0.87, 0.71}5863.26&3555.74 \\ \cline{3-24}
         
     {\textbf{\deftextEsynTurbo}}    & & \textbf{130nm} & 2319.72 & 769.49 &\cellcolor[rgb]{0.77, 0.87, 0.71} 108250.07 & \cellcolor[rgb]{0.77, 0.87, 0.71}1705.39 & 69867.01 & 99645.56 & 50368.3 & 3789.88 & \cellcolor[rgb]{0.77, 0.87, 0.71}42386.9 & \cellcolor[rgb]{0.77, 0.87, 0.71}6104.6 & 130088.52 & 1036197.5 & 10188.52 &\cellcolor[rgb]{0.77, 0.87, 0.71}744.46 & 142655.56 &\cellcolor[rgb]{0.77, 0.87, 0.71} 119931.27 & 3816.16 & 474.2 &\cellcolor[rgb]{0.77, 0.87, 0.71} 10438.76 &\cellcolor[rgb]{0.77, 0.87, 0.71} 24482.23&15780.17 \\ \cline{2-24}

     
  {\textbf{+}}& \multirow{2}{*}{\textbf{lev}}& \textbf{7nm} & 15 & \cellcolor[rgb]{0.77, 0.87, 0.71}10 & \cellcolor[rgb]{0.77, 0.87, 0.71}4977 &\cellcolor[rgb]{0.77, 0.87, 0.71} 3 & \cellcolor[rgb]{0.77, 0.87, 0.71}247 &\cellcolor[rgb]{0.77, 0.87, 0.71} 262 & 57 & 149 & \cellcolor[rgb]{0.77, 0.87, 0.71}87 & \cellcolor[rgb]{0.77, 0.87, 0.71}133 & \cellcolor[rgb]{0.77, 0.87, 0.71}89 & \cellcolor[rgb]{0.77, 0.87, 0.71}24685 &\cellcolor[rgb]{0.77, 0.87, 0.71} 158 & \cellcolor[rgb]{0.77, 0.87, 0.71}19 & 4377 & \cellcolor[rgb]{0.77, 0.87, 0.71}330 &\cellcolor[rgb]{0.77, 0.87, 0.71} 12 & \cellcolor[rgb]{0.77, 0.87, 0.71}6 & \cellcolor[rgb]{0.77, 0.87, 0.71}12 & 160&\cellcolor[rgb]{0.77, 0.87, 0.71}103.19 \\ \cline{3-24}
  
     {\textbf{\textit{{dch}}}}& & \textbf{130nm} &\cellcolor[rgb]{0.77, 0.87, 0.71} 12 & \cellcolor[rgb]{0.77, 0.87, 0.71}10 & \cellcolor[rgb]{0.77, 0.87, 0.71}4977 & \cellcolor[rgb]{0.77, 0.87, 0.71}3 & \cellcolor[rgb]{0.77, 0.87, 0.71}220 & \cellcolor[rgb]{0.77, 0.87, 0.71}262 & 57 & 149 & \cellcolor[rgb]{0.77, 0.87, 0.71}87 & \cellcolor[rgb]{0.77, 0.87, 0.71}193 & 93 & \cellcolor[rgb]{0.77, 0.87, 0.71}24687 & \cellcolor[rgb]{0.77, 0.87, 0.71}148 & \cellcolor[rgb]{0.77, 0.87, 0.71}19 & \cellcolor[rgb]{0.77, 0.87, 0.71}4374 & \cellcolor[rgb]{0.77, 0.87, 0.71}305 &\cellcolor[rgb]{0.77, 0.87, 0.71} 11 & \cellcolor[rgb]{0.77, 0.87, 0.71}6 & \cellcolor[rgb]{0.77, 0.87, 0.71}12 & \cellcolor[rgb]{0.77, 0.87, 0.71}158&\cellcolor[rgb]{0.77, 0.87, 0.71}102.32 \\ \cline{2-24}
     
         & \multirow{2}{*}{ \textbf{Delay($ps$)}}& \textbf{7nm} &\cellcolor[rgb]{0.77, 0.87, 0.71} 108.45 & 80.39 & \cellcolor[rgb]{0.77, 0.87, 0.71}97659.4 & \cellcolor[rgb]{0.77, 0.87, 0.71}69.63 &\cellcolor[rgb]{0.77, 0.87, 0.71} 3003.68 & \cellcolor[rgb]{0.77, 0.87, 0.71}3273.48 & \cellcolor[rgb]{0.77, 0.87, 0.71}828.41 & \cellcolor[rgb]{0.77, 0.87, 0.71}1718.55 & \cellcolor[rgb]{0.77, 0.87, 0.71}941.07 &\cellcolor[rgb]{0.77, 0.87, 0.71} 1049.99 & \cellcolor[rgb]{0.77, 0.87, 0.71}1512.89 & 365492 & \cellcolor[rgb]{0.77, 0.87, 0.71}1756.25 &\cellcolor[rgb]{0.77, 0.87, 0.71} 162.05 &\cellcolor[rgb]{0.77, 0.87, 0.71} 64754.64 & \cellcolor[rgb]{0.77, 0.87, 0.71}4568.78 &\cellcolor[rgb]{0.77, 0.87, 0.71} 126.13 & \cellcolor[rgb]{0.77, 0.87, 0.71}45.62 & \cellcolor[rgb]{0.77, 0.87, 0.71}236.68 & \cellcolor[rgb]{0.77, 0.87, 0.71}2695.16&\cellcolor[rgb]{0.77, 0.87, 0.71}1280.34 \\ \cline{3-24}
         
         & & \textbf{130nm} &\cellcolor[rgb]{0.77, 0.87, 0.71} 685.26 &\cellcolor[rgb]{0.77, 0.87, 0.71} 495.47 & \cellcolor[rgb]{0.77, 0.87, 0.71}458235.06 & \cellcolor[rgb]{0.77, 0.87, 0.71}402.39 &\cellcolor[rgb]{0.77, 0.87, 0.71} 12147.18 & \cellcolor[rgb]{0.77, 0.87, 0.71}17216.68 & \cellcolor[rgb]{0.77, 0.87, 0.71}4196.77 & \cellcolor[rgb]{0.77, 0.87, 0.71}8982.54 &\cellcolor[rgb]{0.77, 0.87, 0.71} 4435 &\cellcolor[rgb]{0.77, 0.87, 0.71} 8243.77 & \cellcolor[rgb]{0.77, 0.87, 0.71}7714.58 &\cellcolor[rgb]{0.77, 0.87, 0.71} 2243522.25 & \cellcolor[rgb]{0.77, 0.87, 0.71}10527.65 & \cellcolor[rgb]{0.77, 0.87, 0.71}1022.69 &\cellcolor[rgb]{0.77, 0.87, 0.71} 319666.91 &\cellcolor[rgb]{0.77, 0.87, 0.71} 23086.99 & \cellcolor[rgb]{0.77, 0.87, 0.71}789.4 & 362.24 & 1421.45 &\cellcolor[rgb]{0.77, 0.87, 0.71} 12811.74&\cellcolor[rgb]{0.77, 0.87, 0.71}7170.83 \\ \cline{2-24}

         
        & \multirow{2}{*}{\textbf{runtime($s$)}}& \textbf{7nm} & 3.61 & 6.29 & 22.8 & 5.17 & 15.82 & 27.83 & 11.9 & 7.86 & 17.76 & 7.8 & 29.11 & 1118.53 & 5.79 & 4.58 & 44.85 & 44.24 & 5.6 & 3.168 & 6.16 & 16.64&13.61 \\ \cline{3-24}
         & & \textbf{130nm} & 3.76 & 3.84 & 26.48 & 2.42 & 13.7 & 18.48 & 5.75 & 3.17 & 11.12 & 2.11 & 36.74 &\cellcolor[rgb]{0.77, 0.87, 0.71} 717.47 & 1.92 & 3.975 & 29.11 & 27.74 & 1.78 & 1.31 & 3.61 & 4.85&7.78 \\ \hline
    \end{tabular}}
\end{table*}
